Reinforcement Learning based Proactive Control for Transmission Grid Resilience to Wildfire

Power grid operation subject to an extreme event requires decision-making by human operators under stressful condition with high cognitive load. Decision support under adverse dynamic events, specially if forecasted, can be supplemented by intelligent proactive control. Power system operation during wildfires require resiliency-driven proactive control for load shedding, line switching and resource allocation considering the dynamics of the wildfire and failure propagation. However, possible number of line- and load-switching in a large system during an event make traditional prediction-driven and stochastic approaches computationally intractable, leading operators to often use greedy algorithms. We model and solve the proactive control problem as a Markov decision process and introduce an integrated testbed for spatio-temporal wildfire propagation and proactive power-system operation. We transform the enormous wildfire-propagation observation space and utilize it as part of a heuristic for proactive de-energization of transmission assets. We integrate this heuristic with a reinforcement-learning based proactive policy for controlling the generating assets. Our approach allows this controller to provide setpoints for a part of the generation fleet, while a myopic operator can determine the setpoints for the remaining set, which results in a symbiotic action. We evaluate our approach utilizing the IEEE 24-node system mapped on a hypothetical terrain. Our results show that the proposed approach can help the operator to reduce load loss during an extreme event, reduce power flow through lines that are to be de-energized, and reduce the likelihood of infeasible power-flow solutions, which would indicate violation of short-term thermal limits of transmission lines.

==> 0_overview.tex <==

% \subsection{Overview and RL Algorithm}
% {\color{red}Describe RL approach semi-formally in terms of the model (we do not need to describe DDPG and whatever other algorithms we use in detail, we can provide high-level idea and references).}



We want an agent that will be able to make the right decision proactively at the right time based on the current state of the environment. To make the right decision, the agent satisfies several constraints (described in the model) in its action and the action minimizes the weather impact. We can have such an intelligent agent by training it properly for that environment. 


\subsection{Overview}
To train the agent, we develop a test environment that simulates the fire propagation model and the power system model. The agent makes the decision and interacts (action) with the environment at every time step based on the information (observation) that it gets from the environment.


\subsubsection*{Power system operator}
The power system needs to maximize its efficiency. It aims to maximize the power generation to reduce the load loss and distribute it efficiently. We use GAMS as power system operator to solve the optimization problem. 


\subsubsection*{Simulator}
On top of the power system operator, we implement a simulator. The simulator simulates the external weather and interacts with the power system operator. We simulate fire as an external calamity. When the fire reaches any component of the power system, the simulator tells the system operator to shut off the buses or branches. 


\subsubsection*{Agent}
The simulator can not take any action proactively. To take an action proactively, we build an RL agent. Based on the external weather information provided by the simulator, the agent tells the system operator to ramp up/down the power generation of generators and shuts off buses or branches proactively before reaching the fire. 




==> 1_introduction.tex <==
\section{Introduction} 

\IEEEPARstart{R}{ecent} statistics~\cite{USbillion-dollar} show that the frequency of extreme weather events (also classified as high impact low frequency, or HILF, events), such as storms, floods, and wildfires, and associated impact on the power grid have soared up in recent years. While each of these different kinds of weather events comes with its own subtleties, one aspect is common: infrastructure destruction and multiple faults leading to catastrophic failure of the power system \cite{7105972}. Following a fast-moving disaster striking the power system assets, especially, in the case of hurricanes, snowstorms, typhoons, windstorms, floods, lightning storms, the component failure rate varies with the intensity of hazardous forces \cite{7434044}. Contrarily, the wild-fire events are relatively slow progressing event \cite{7105972}, and directly affects the flow through the transmission lines \cite{CHOOBINEH201520}. 

Once the fire-hazard encroaches the power system, especially distribution system, it will have disastrous impact on the non-fire hardened poles, cross-arms, insulators, and uncovered conductor wires. \Aron{this sentence is still convoluted (first part states that unlike other disasters, glass fires can have impact not only poles, cross-arms, etc., but it does not state what else glass fires may impact, which is supposed to be the key message of the first part; second part states that wild fires can originate from vegetation blown into transmission lines, which is a mostly unrelated aspect (impact vs. origin))}\Subir{I meant to state here the importance of Wildfires compared to other natural disasters. Power lines can also be the origin of wild fire, which is not true for other kind of disasters.}
Furthermore, contrary to other weather related events, in an intensely heated surrounding, high winds can blow nearby vegetation into the transmission lines, which can create sparks, snap transmission lines with the potential of originating the wildfire hazard \cite{Western.2021}. This gained additional significance for the wildfires in the recent years; and has motivated some utilities in the USA to restrict the power flow through some of their assets (e.g., public safety power shut-off, or PSPS, events in the state of California, USA) \cite{abatzoglou2020population}. Therefore, unlike other events where the major focus is on disaster planning and restoration, more focus is needed for power system operation control and management in case of wildfires. While scope this work is limited to controlling power system proactively given an already progressing wildfire, it remains silent on its origin, i.e., directly prohibiting wild-fire event to originate from power system due to the lack of modeling detail. This will be one of the scope of our future work.

\subsection{Literature Review} 
For effective management of power system operation, in addition to obtaining a better prediction of outage risk, emergency control actions need to be planned proactively, continuously monitored, and the actions of generating entities, independent System Operators / regional transmission operators, distribution system operators, aggregators, load serving entities, need to be properly coordinated among various entities within the electric grid. Availability of abundant monitoring data from SCADA and PMUs along with the pre-event abundance of human inference can be leveraged in this regard \cite{ji2016large}. In this regard, several statistical outage duration models \cite{doi:10.1061/(ASCE)1076-0342(2005)11:4(258), 6949604, nateghi2014forecasting} can be referred to, which can help operators determine the desirable proactive measures to reduce the imminent outage duration. 

Since, the propagation of these weather events can be treated as a stochastic process, traditional multi-period stochastic optimization can be useful in this regard. However, computational complexity poses a significant challenge to its deployment. Alternatively, one can rely on these forecasts for carrying out the deterministic multi-period optimization, reducing computational complexity significantly. However, due to the combinatorial nature of the solution space, especially with optimal transmission reconfiguration and generation commitment and scheduling \cite{1372745,4162603,ahmadi2014distribution}, it is difficult to perform multi-period optimization in real-time. Furthermore, some of these coordinated control actions need to be planned several hours ahead. Since forecasts can be inaccurate in the longer operating time horizon, the associated proactive plan needs to be readjusted as and when required. Machine learning (ML)-based techniques, suitably trained apriori based on the available measurements, can be leveraged to significantly reduce the computation time while offloading the majority of the decision making onto the computer, resulting in a fast and efficient decision-making \cite{7951075}. This alleviates the discussed difficulties of proactive optimization and rule-based approaches while minimizing the possibility of imminent human errors due to operating in a stressful environment.


%In the advent of imminent disaster, often to limit catastrophic failures originating from the electricity transmission assets themselves, the power flow through some of the assets needs to be restricted (e.g., PSPS events in the state of California, USA)


\Aron{some of this text could be moved to a related work section since this is not necessary to understanding our approach and its context}
\Subir{Pls. Chk}
 
% \Aron{this transition also needs to be more smooth, paper suddenly starts talking about prediction, this needs to be motivated}
% In this regard, the use of negative binomial regression for accurate prediction of outage duration based on a large GIS database of three hurricanes (namely, \Aron{we need to turn these into proper references}Floyd (1999), Bonnie (1998), and Fran (1996)) has been developed in \Aron{how is this reference related to the three earlier in the sentence?}\cite{doi:10.1061/(ASCE)1076-0342(2005)11:4(258)}. 
% However, such a developed model is specific to a given geographic area. A hurricane outage prediction model applicable along the entire U.S coastline has been developed in \cite{6949604}. Another statistical outage duration model has been developed in \cite{nateghi2014forecasting}, while validating this model against the events resulted in a \Aron{``central Gulf Coast states''? i.e., Louisiana, Mississippi, and Alabama?}central gulf coast state. 
% These statistical models can help the operators to determine the desirable proactive measures to reduce the imminent outage duration. 

% In addition to the possible utilization of historical measurements, machine learning-based approaches can also utilize realistically generated artificial datasets using simulators following similar probabilistic structure but requiring no real-world measurements. Such a combined approach can drastically improve the sampling efficiency to generate a pre-trained model. Additionally, although these ML-based approaches are expected to work in a simulated environment, the use of an artificial dataset can easily identify some of the maloperations that may lead to cascading, which the traditional methods will not be able to identify. \Aron{is this relevant to our paper?} \Subir{If deemed not necessary, please remove.} 

The use of machine learning approaches for improving the power system resiliency is also abundant. The use of the generative adversarial network (GAN), a data-driven ML approach, that utilizes PMU-data while simultaneously generating missing data utilizing a  deep neural network for the pre-fault dynamic security assessment (DSA) with high accuracy and lower computational complexity is observed in \cite{8736295}. The use of deep-reinforcement learning for the power system emergency control has been discussed in \cite{huang2019adaptive} and the Q-learning framework has been utilized in this regard. Machine learning techniques have also been utilized for determining expected potential load curtailment within the grid. In this regard, \cite{7752978} uses logistic regression, and \cite{eskandarpour2019probabilistic} uses a combination of a twin support vector machine model, posterior probability sigmoid model, and probabilistic load curtailment estimation model. Therefore, the existing rich literature on power system decision support and recent advances in ML-based control \cite{KHARGONEKAR20181} indicates the possibility of successful deployment of ML-based techniques for proactive control of the power system in the advent of a disaster. 

The use of traditional proactive control strategies for the power system resiliency improvement are also abundant, and a detailed literature review is available in \cite{8894433}. Since the control of generating stations and proactive switching of the transmission network is a major concern in our work, we limit our literature review to the transmission network operation. In this regard, a Markovian model of typhoon propagation and fragility of transmission lines in its path has been considered for proactive sequential re-dispatch of generators for resiliency maximization in \cite{wang2016resilience}. Proactive splitting the grid into islands in the advent of HILF events to reduce potential cascading outages while facilitating system restoration has been discussed in \cite{biswas2020proactive}. The use of the transmission system reconfiguration for resiliency improvement has been discussed in \cite{8053185}. In the event of islanding, the coordination strategy of multiple microgrids to exchange power through the transmission network as a resiliency measure is discussed in \cite{7857787, 7127029}. Use of predicted wildfires propagation path into an early warning signal for the transmission system outage has been considered in \cite{8620983} and is one of the major talking points among the power utility companies in the USA \cite{BCG2020}. As already indicated, as the fire encroaches on an energized transmission line, the power flow through it needs to be dynamically modified on a proactive basis. The models for derating power transmission lines are available in \cite{CHOOBINEH201520,10.1007/978-3-662-48768-6_139}. 

\subsection{Problem Statement} 
Since distribution networks are the primary load center and the survival of customer loads is the primary concern of resiliency improvement strategy, majority of the existing proactive operational control strategies revolve around controlling the operation of the distribution network. Local distributed energy resources, microgrids, and deployment of moving diesel generators facilitate such treatment. However, as already discussed, since the bulk of the power still flows through the transmission network, and the operation of transmission and distribution network needs to be coordinated, transmission network flows need to be controlled as well. To achieve this, our focus here is limited to optimal proactive flow and topology control of the power transmission network. We will seek the help of reinforcement learning as a part of the decision making helping us to reduce the burden on the system operator during critical decision making in a stressful environment. Control of distribution network and integrated transmission and distribution network control will be the focus of our future work.


% \textcolor{red}{In this section, we present a DRL based agent that supplement a reactive system operator to better manage the grid during wildfire propagation. The agent aids the operator by recommending actions pro-actively to minimize the impact of wildfire on the grid operations. These actions include removing power system equipment or changing power injections at some nodes in the system. Our approach is based on Deep Reinforcement Learning (DRL) that aims at training a neural network to learn a policy which maximizes the expected reward, (Equation~\ref{eq:total}) in an \textit{offline} setting. A trained agent can generate preventive actions without any computation overhead in real time as opposed to \textit{online} multi-step stochastic optimization techniques~\cite{2015paper} that solve time consuming and computationally very expensive optimization problems on demand at run time. }

% Consequently, although the recent literature shows the abundance of recent literature on preparing the distribution network before an imminent disaster, associated work on the power transmission network, along with transmission distribution coordinated resiliency improvement is \Aron{in what way? what is missing? what are the key challenges?}sadly limited. However, the bulk power still flows through the transmission network; and the operation of transmission and distribution network should be coordinated. 


%Although the recent literature shows the abundance of recent literature on preparing the distribution network before an imminent disaster, associated work on the power transmission network, along with transmission distribution coordinated resiliency improvement is \Aron{in what way? what is missing? what are the key challenges?}sadly limited. Furthermore, the initial result of the application of machine learning approaches for power system resiliency improvement shows promising result, application of machine learning techniques for active control of generating and transmission assets for resiliency improvement is also limited. 

Since the developed Reinforcement Learning (RL) agent is the primary decision making entity, the activity of the power system operator majorly becomes reactive. Here, the agent provides the system operator with a partial set of control actions. The operator, based on the current observation, security status of the system, prediction of the state of next time period, and partial control action set from the agent generates the entire control signal, and deploys it into the power system. Given that the spatio temporal fire growth dynamics to be a Markovian process \cite{BERTSIMAS2017664}, and the reactive power system operator, the RL-agent need to be suitably trained, and a test-bed need to be developed in this regard. The developed test-bed allows us with an in-policy training of the developed RL agent. A detailed description of the model and the agent can be found in Sections \ref{sec:model} and \ref{sec:Formulation}. The initial result shows that $\cdots$\Himanshu{TODO:}

% To solve these challenges, assuming that the spatio temporal fire growth dynamics to be a Markovian process \cite{BERTSIMAS2017664}, and typical corrective transmission system operation, we have developed an integrated framework for the co-simulation of wildfire propagation and power system operation. Here, we have assumed that the wildfire propagation and the transmission system operation are independent processes. Both these processes interact when the active fire interacts with energized transmission lines, generators, or generating/distribution substations. Consequently, the power system operator obtains input from both the trained ML-based external agent and the wildfire environment (exogenous variables). The ML-based external agent may control all/partial sets of generators and transmission lines. The myopic operator within the power system operational environment optimally allocates resources (if the external agent controls a partial set of generators) to ensure continuous balancing of the supply and demand (endogenous parameters). The operator also determines the need to shed loads. The actor-critic framework of the reinforcement learning (RL) approach has been utilized for training the external agent. A detailed description of the model and the agent can be found in Sections \ref{SecModel} and \ref{SecFormulation}. The initial result shows that $\cdots$

%Be Technical about it. Provide an overview

\subsection{Contributions}
In this paper, we developed a novel approach and an associated simulation testbed for effective power system operation control and management in the presence of wildfires. The core contributions of this paper are as follows:
\begin{itemize}

\item[(i)] Integration of the wildfire and power system models. \Himanshu{TODO: elaborate}

\item[(ii)] Formulation of the decision problem as a MDP. Describing the rewards and costs. \Himanshu{TODO: elaborate}

\item[(iii)] Integration of the simulation frameworks in a unified testbed. \Himanshu{TODO: elaborate}

\item[(iv)] Solving the MDP using DDPG. \Himanshu{TODO: elaborate}

\end{itemize}

%%Himanshu: Commenting out the old statements.. Added the contribution statement above. Tbe listed contributions need elaboration.
%Contributions of this paper are threefold:
%\begin{itemize}
%\item[(i)] Integrated Test-bed development (elaborate)
%\item[(ii)] RL framework development (elaborate) 
%\item[(iii)] Performance of our approach (elaborate) 
%\end{itemize}

\subsection{Paper Organization}
The remainder of the paper is organized as follows. The model for the propagation of wildfire, proactive control of the power system, and the integrated co-simulation environment are described in Section II. The formalization of the reinforcement learning problem is discussed in Section III. The description of the agent, complexity analysis, and training framework is discussed in Section IV. Section V presents simulation results and performance of the algorithm. Sections VI concludes the paper.


% \textcolor{red}{Pl. ignore next three paragraphs. I am editing now. Will be ready tonight}
% Aggregating these factors, a model that determines the impact of wildfires on the line tripping is considered in \cite{petrovic2012dynamic}. 
% Furthermore, when the fire breaks out, the necessity of suppressing the wild-fire automatically arises, and, suppression probability also impacts its effect on transmission lines; and a dynamic resource allocation for the suppression of fire is considered in \cite{shi2018model}, which is required to be carried out alongside resource allocation to reduce the impact of fire-hazard on the transmission lines in a limited resource disaster scenario. Furthermore, wild-fire is often coupled with heat waves, during which the peak load demand flowing through those transmission lines remains quite high \cite{CHOOBINEH2016230}; along with this the growth in ninetieth percentile peak load demand is also on the rise \cite{sathaye2011estimating}. Increasing peak demand coupled with reduced line rating increases the risk of unserved load and load shredding. Local provision of power from distributed generators can reduce the risk of load shredding during these events and stochastic programming approach has been utilised in \cite{doi:10.1002/etep.2043, 6939103} for optimal resource allocation. Like transmission network, because of lower clearance height, distribution network too can suffer from failure, requiring reconfiguration on network lines, which is also considered in \cite{7995099} for decision-making. However, since the proactive action needs to be taken beforehand, and the severity of wild-fire is not known a priori, a stochastic mathematical programming problem has been introduced in \cite{MOHAGHEGHI2015843}. 

% It is well known that local provision of power not only reduces reliance of the distribution network on transmission network, the presence of active component also allows the distribution network to be operated as islanded microgrids in the aftermath of a disaster \cite{4762177}; and distribution system reconfiguration facilitates that \cite{6202397}. Boundary of microgrids formation can be fixed or dynamic. In a microgrid with fixed boundary, although the microgrid is designed to operate in a grid connected mode, it is configured to operate as an island \cite{1626398}. Microgrid, that are formed by strategic operation of switches, their boundary is entirely driven by automated reconfigurable feeder switches, and is therefore flexible. While, most of the literature assumes the presence of renewable energy resources; their variability, especially during the disaster poses significant challenges, forcing us to use battery storage devices. As indicated in the earlier reported works, operation as a microgrid in the aftermath of a wildfire damaging distribution network is also widely considered topic. Coordinated operation of combination of microgrids has the potential to significantly reduce electricity outage during extreme events \cite{barnes2017tools}. A novel sequential restoration of electricity supply through coordination among multiple microgrids has been proposed in \cite{doi:10.1002/etep.404}. Nevertheless, it is well known that because of switching operation requirement, the restorative reconfiguration problem is combinatorial in nature \cite{1372745,4162603,ahmadi2014distribution}; and it is difficult to solve a large dimentional problem with integer variables because of computational intractability \cite{7101299}. Nevertheless, formation of multiple microgrid following natural disasters through distributed multi-agent communication has been considered in \cite{7127029}. It is important to note that the work reported until now remains silent about the sequence of switching operation; however, they are increasingly being considered in the recent literature, especially for the active interfaced distribution network. In this regard, a spanning tree search-based algorithm is utilized in \cite{6781027} to obtain switching sequence for power system restoration.  A multi-time step sequential service restoration framework is developed in \cite{7971935}. Selection of the restoration sources and formation of microgrids along the restoration paths has been considered in \cite{5759139} to reduce the congestion level during restoration. Multi-agent system based service restoration though controlled islanding using distributed generators has also been considered in \cite{7088641}. Cooperative decentralised multiagent framework for restoration with multiple distribution network is considered in~\cite{6205352}.


% \Aron{this sentence is already included earlier}While each of the different kinds of weather events come with their own subtleties, one aspect is common; that is infrastructure destruction and occurrence of multiple faults due to catastrophic damage \cite{7105972}; and thus, helplessness of protection devices to clear the fault. Like, `after a storm comes a calm', and within that period of calmness it is important to restore the network so that our heavily electricity infrastructure-reliant society reach to a new normal. While one approach could be remote operation of reconfigurable switches, which can be used to restore the network without physical crew deployment, because of infrastructure damage it becomes necessary to deploy the crews. Situation becomes further worsened, if the natural disaster occurs during the pandemics, such as COVID-19, where social distancing becomes essential. It is also important to know that unlike fast progressing natural events (e.g., Tsunami, Tornado, Hurricane, Blizzard, Earthquake), which often takes from hours to days to complete, wild-fire is a slow progressing event \cite{7105972}. Therefore, during such slow progressing event, depending on the movement of the wild-fire crews has sufficient chance of propositioning itself so that the damages can be repaired at the soonest. While there can be many ways to gather information about system damage, finite availability of resources require jobs to be prioritized. Since multiple of damage repair requests needs to be handled simultaneously, myopic decision policies for ERM can be inefficient, and in this regard decentralised multi-agent Monte-Carlo Tree Search method \cite{claes2017decentralised} can be essentially useful.


\Aron{need to add (1) summary of contributions and (2) paper outline (combine them if there is not enough space)}

==> 2_environment.tex <==
\section{Modeling Impact of Wildfire on Power Grid Performance
%Modeling Power Grid Performance Impact of Wildfires
}\label{SecModel} {\color{red}[3 pages]}

\Aron{add introductory paragraph, providing very brief overview of this section (i.e., elements of our model and perhaps high-level assumptions, such as discrete time)}

\Aron{add figure showing the model (including agent and real environment)}

%Just state about the combined model. Don't go into details. Reserve the details for later.

As indicated earlier, the load-generation balance needs to be continuously ensured within the power system, and the power system operator continuously strives to ensure the same. Regulation services handle the rapid fluctuation of loads. Allocation of sufficient load-following reserve can help mitigate intra-period slower fluctuation, and the operator needs to ensure the establishment of set-points for the generators for each of the periods \cite{doi:https://doi.org/10.1002/0470020598.ch5}. Consequently, the operating horizon becomes highly discretized, and a quasi-static model has been considered here. Additionally, here the primary focus is on the slow cascading phase where the stability of the power system is not directly thwarted \cite{HENNEAUX201241}. If one of the lines is tripped due to overloading, unless the flow is proactively controlled, it is imminent that adjacent lines will be overloaded. Subsequently, the transmission lines will trip like a domino, and hence cascading will occur. 

The fire propagation environment is similarly discretized by \Aron{what else is split into cells?} splitting the fire propagation environment into cells. \Aron{these details should go into the subsection}Each of the cells contains a certain amount of fuel resource. Depending upon the state of neighbouring elements, a cell can catch fire with a certain probability. Furthermore, once caught on fire, the fuel burns until it gets exhausted. The temporal horizon of the fire propagation is also discretized. While the selection of a larger spatiotemporal grid would speed up the simulation of the fire-propagation model, it would significantly reduce model accuracy \cite{}\Himanshu{TODO}. 

To enable the cosimulation of wildfire propagation and power system operation, the power transmission system is geocoded, and the wildfire and the power system only interact if wildfire trips any of the transmission lines, generating/distribution substation, and power generators. Detailed description of the wildfire propagation and the power system model and their interaction is provided in the following subsections. 

\Aron{add table listing symbols used throughout this paper (if we have space)}

\subsection{Modeling Wildfire Spread}

\Aron{this needs to be written up into a proper paragraph of sentences}

\Aron{more importantly, we first need to (1) introduce the concept of cells (and their properties) and (2) state that our model is discrete time}
{\color{red}Formal model of wildfire spread.}\\
\input{fire_spread}

\subsection{Modeling Impact on the Power Grid and Proactive Control Actions}
{\color{red}Formal model of power grid (I guess that we can reference prior work heavily here to save time and space).}

\Aron{please add some paragraph headers to this subsection to improve readability}

As indicated earlier, the system operator's primary objective is to ensure that load and generation are always satisfied for each time period while avoiding cascading outages. Consequently, these four key constraints must be satisfied at all times to ensure the normal operation of the entire power system: (i) non-violation of the thermal rating of electric transmission equipments, (ii) ensuring maintenance of the voltage within desired limits, (iii) ensuring load-generation balance (satisfying the physics of the power system), and (iv) operational constraints of generating resources in regards to their ramping up and down capability. The system operator's primary objective here is two-fold: (i) to minimize the impact of external weather events on the electricity loads, thereby minimizing the load shedding, and (ii) operate transmission, distribution, and generating equipment in such a way that a disaster cannot take out any energized device, thus minimizing the chances of cascading (since the chances of line tripping due to hidden failures cannot be eliminated \cite{THORP1998147}). 

% Additionally, in order to prohibit weather events from directly affecting the transmission assets, one should also not take out any energized transmission lines apriori. Furthermore, the power flows through transmission equipments from the generating station to the distribution network, connected at various nodes of the transmission system, to satisfy the load demand while following the laws of physics.  We assume the presence of sufficient rotational inertia and reserve (not directly accounted for here) so that even when generators ramps up or load fluctuates, load-generation balances are always maintained. 

An electric power system comprises a finitely many nodes (generating or transmission substations), $V_t$, and edges (transmission lines), $E_t$. The nodal and transmission line availability is a function of time, depending upon the isolation of energized substations and transmission lines. Following the model's discussed quasi-static nature, we assume that the number of buses and edges within a given discretized period remains constant (except at the beginning of a period when the switching is being conducted). Additionally, during each of the operating period, both generation ($P^G_{i,t}$) and loads ($P^L_{i,t}$) are assumed to be constant. For simplicity, we assume that multiple available generating resources at a given node are aggregated. Since the typical operating voltage within the power system remains close to 1.00 \textit{pu}, and the difference in the voltage angle ($\theta_i$) of the adjacent buses are very small, we consider a DC power flow model. Here, the DC power flow equations determine the power flow directions through transmission lines (driven by physical laws). The voltage angles are also bounded by $\underline{\theta}$ and~$\overline{\theta}$.

The loads within the distribution network can be categorized based on their criticality. If one of the lines is outaged (determined by, $\delta_{i,j,t}$) following the instruction of the external agent or due to the operation of circuit breakers, the flow needs to be redistributed, forcing the generators to ramp up/down. If the desired output is beyond the capability of a generating and transmission resource, we need to shed some of the load. The load shedding ($\Delta P^{C,L}_{i,t}$ and $\Delta P^{NC,L}_{i,t}$) is dependent upon the criticality (availability of power to hospitals, police stations, fire stations, etc., are much more important than residential demand), and is limited by an associated fraction ($\alpha_i$). Availability of a large number of loads within the distribution network that is connected at the transmission substation enables treating the sheddable loads as a continuous variable. Additionally, as indicated earlier, the generation outputs are limited by associated power generation upper and lower limits ($\overline{P^G_i}$, $\underline{P^G_i}$), and ramp-rate limits ($\underline{\mathcal{R}(i)}$ and $\overline{\mathcal{R}(i)}$). Since up- and down-time are generally driven by economic concerns, those limits have been ignored here. Here, $i$, and $t$ represent nodes of the power system and time intervals, respectively. Consequently, the equations driving power system operation can be given by the following set of equations:

\begin{gather}
    P^{G}_{i,t+1}  - P^L_{i,t+1} + \Delta P^{C,L}_{i,t+1} + \Delta P^{NC,L}_{i,t+1} - \sum_i P^{Line}_{i,j,t+1} = 0 \label{Node_Bal} \\
    P^{Line}_{i,j,t+1} - \left( \theta_{i,t+1} - \theta_{j,t+1} \right ) B_{i,j} \delta_{i,j,t+1} = 0 \label{Power_Flow_01} \\
    \underline{\theta} \leq \theta_{i,t+1} \leq \overline{\theta} \label{angle_lim} \\
    0 \leq \Delta P^{C,L}_{i,t+1} \leq \alpha_i P^L_{i,t+1} \label{Crit_lim}\\
    0 \leq \Delta P^{NC,L}_{i,t+1} \leq (1 - \alpha_i) P^L_{i,t+1} \label{NCrit_lim}\\
    \underline{P^{Line}_{i,j}} \delta_{i,j,t+1} \leq P^{Line}_{i,j,t+1} \leq \overline{P^{Line}_{i,j}}\delta_{i,j,t+1} \label{line_therm}\\
    \underline{P^{G,n}_{i}} u_{i,t+1} \leq P^{G,n}_{i,t+1} \leq \overline{P^{G,n}_{i}} u_{i,t+1} \label{Gen_lim}\\
     - M u_{i,t+1} + k_h\underline{\mathcal{R}(i)} \leq P^{G}_{i,t+1} - P^{G}_{i,t} \leq k_h\overline{\mathcal{R}(i)}  + M u_{i,t+1} \label{ramp_lim}\\
    u_{i,t+1} \leq \psi_{i,t+1} \wedge u_{i,t} \\
    \psi_{i,t+1} = \left\{\begin{matrix}
1, & i \in V_{t}\setminus \left( \Delta V_{t} \cup \Delta' V_{t}\right ) \\ 
0, & \text{otherwise}
\end{matrix}\right. \label{bus_avl}
\end{gather}

The polytope representing the power system event space, as given in \eqref{Node_Bal}-\eqref{bus_avl} (also given by $\Phi_{t+1}$), determine temporal evaluation of the system. The decision variables are driven by, $DV = \lbrace \bm{P^{G}_{t+1}}$, $\bm{\Delta P^{C,L}_{t+1}}$, $\bm{\Delta P^{NC,L}_{t+1}}$, $\bm{P^{Line}_{t+1}}$, $\bm{\theta_{t+1}}$, $\bm{u_{t+1}} \rbrace$. Line operating conditions determined from $\delta_{i,j,t+1}$ can be obtained from either the fire-model or the system operator. If the solution to these set of equations does not exist, then it is imminent that primarily either the load generation balance is not satisfied (given the generator set-point during the previous period), or the thermal rating of the lines is violated. We assume that power plants are equipped with load rejection capabilities \cite{4111968}. Therefore, the sudden outage of a substation will not impact the rest of the power system operation; and such a condition should not lead us to an empty set. This is achieved utilizing the big-M approach in \eqref{ramp_lim}. Once a generator is outaged, it will not be up until there is no fire threat, and the operator manually brings it online. The fire threat and the availability of a generator is given by $\psi_{i,t+1}$ and $u_{i,t+1}$, respectively. Also, $\Delta V_{t}$ and $\Delta' V_{t}$ denotes substation removal command by the agent and due to circuit breaker operation, respectively.

If the solution to these set of equations exists, given a set of observation, the system operator would isolate the threat first (through $\delta_{i,j,t+1}$ and $\psi_{i,j,t+1}$), and provide set-points to the generators to minimize the load to be shedded for the next period, while minimizing the ramping up of generators. As indicated earlier, in the event the exogenous agent decides to control a subset of generators, output from the remaining set of generators can also be controlled by the system operator. As opposed to the traditional approach, where the forecast of multiple time periods in the future is available to the operator, the system operator considered here is myopic to the operating state during the next time period. Consequently, the operational objective of the power system, as decided by the system operator, can be given by:

\begin{equation}
    s^\textit{power}_{t+1} = \arg \min_{DV} \begin{Bmatrix}  \rho^C \bm{\Delta P^{C,L}_{t+1}} + \rho^{NC} \bm{\Delta P^{NC,L}_{t+1}} \\
   \left. + \epsilon || \bm{P^{G}_{t+1}} - \bm{P^{G}_{t}} ||^2_2 ~~~\right| \Phi_{t+1}  \end{Bmatrix}
\end{equation}

The selection of sole minimization of the value of lost load objective by the system operator would lead to multiple possible solutions, and some of these possible solutions would lead to undesirable ramping up and down of some of the generators. Incorporation of $\epsilon || \bm{P^{G}_{t+1}} - \bm{P^{G}_{t}} ||^2_2$ in the objective function, where $\epsilon$ is a small positive real number, would discount such undesirable conditions, with little to no impact on our minimal value of loss of load objective. Since the system operator considered here is myopic, the agent considered here aims to replace the system operator's traditional multi-period decision-making requirement through implicit prediction of the future state and determining the best course of action to be taken now to minimize the impact of future disaster. 

\subsection{Model Integration Architecture}

\Aron{?}

==> 2_environment_aj.tex <==
\section{Model and Problem Formulation}
\label{sec:model}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/pics/blockdiagram.pdf}
    \caption{System Block Diagram }
    \label{fig:blockdiagram}
\end{figure}

Figure~\ref{fig:blockdiagram} shows the block diagram of the system model that captures the propagation of wildfire in a landscape, power system operations and the impact of the wildfire on the power system equipment and operations based on discrete \sout{model of }time \addtxt{model}. The system model consists of three major blocks labeled as: \Subir{Change the block diagram according to the revision. Successively, Fig. 3 will also be changed. Seek where you are gathering the information from the wild-fire simulator, and update that accordingly.}
\begin{itemize}
    \item \textbf{$\mathcal{F}^{fire}$}: This is a stochastic function that represents the spreading of fire in a region. \addtxt{Due to its inherent Markov property, the internal } \sout{The }output of the function depends solely on the state of the wildfire in the previous time step, \change{$s^{f}_{k-1}$}{$s^{f}_{n-1}$}. \addtxt{This function can operate in a faster timescale compared to rest of the part of the system, by a factor of $\mathbb{D}$; and consequently, the signal is downsampled to obtain the fire propagation observation space, $s^{f}_{k}$.} 
    \item \textbf{$\mathcal{F}^{map}$}: This \change{function models}{is a functional model to represent} the impact of wildfire on the \sout{topology of the} power system operation. It takes the state of wildfire in the region, $s^{f}_{k}$, as the input and produces a local control input, $u^I_k$ (a boolean vector), representing \addtxt{emergency} status of power system equipments\change{ i.e. whether the equipment is operational or not as a result of the proximity of wildfire to the physical location of the equipment.}{. The measurement of this status vector is often indirect, and is obtained from emergency call from the generating and transmission substation or thermal overload condition of the transmission lines \cite{ltmABB} based on temperature measurement, indicating proximity of the encroaching wildfire.}
    \item \textbf{$\mathcal{F}^{power}$}: This block mimics the behavior of \change{ ensure that the value of power system operator that finds an optimal load flow such that}{a reactive and myopic power system operator that seeks the help of an external agent (if available) to find an optimal power flow solution while ensuring minimal value of} load loss at the next (${k+1}^{th}$) step \change{is minimized while considering the current state of the power system,}{. To achieve the same, the operator considers previous state of the power system,} $s^{p}_{k}$, and \addtxt{and the} control inputs, $u^{I}_k$, $u^{E}_k$ (internal and external). The external control input includes \change{changes in generator power levels and}{generator dispatch set-points and active} de-energization of power system equipments.   
\end{itemize}
The mathematical formulation of these functional blocks are defined in following sub-sections with a complete list of notations summarised in Table~\ref{tab:symbols}.

\subsection{Assumptions} \label{2.Assumptions}
\addtxt{The discussed} system model depends upon the following assumptions: (1) \change{Wildfire propagation model assumes the effect of geographical factors such as terrain slope and type along with environmental factors such as wind velocity and humidity etc are}{the geographical and environmental factors are} implicitly captured by \addtxt{the wildfire propagation transitional probability} and is known \change{before hand}{apriori}; (2) \change{The power system operations model assumes the load demand at every node remains constant.}{the power system operator internally estimates the forecast of the load demand, to calculate generator set-points at the next time interval for ensuring system-wide load-generation balance,} \addtxt{(3) availability of sufficient load-following reserve can help mitigate intra-period slower fluctuation \cite{doi:https://doi.org/10.1002/0470020598.ch5} maintained}, \addtxt{(4) slow cascading phase (driven by the transmission line short time overloading) \cite{HENNEAUX201241}, where the stability of the power system is not directly thwarted, is of concern here,} 
\addtxt{(5) the selection of a larger spatiotemporal grid would speed up the simulation of the fire-propagation model, at the expense of significant reduction in the model accuracy \cite{boychuk2009stochastic}, therefore, it is assumed that the fire propagation model operates in a faster time scale, and result of the simulations are appropriately down-sampled,} \addtxt{(6) the state of the power system constitutes of individual state of the generators, operating condition of the loads, transmission and generating stations, transmission lines, along with existence of feasible solution space (non-existence of feasible solution space indicates given generating and load constraints, it is impossible to ensure load-generation balance without violating thermal limit of the transmission lines, indicating cascading failure)}, \addtxt{(7) while possibility of cascading outage cannot be prohibited \cite{THORP1998147}, recovery of the system following cascaded outage condition is not within the scope of this problem}, \addtxt{(8) the delay in measurement of the state and deployment of the control action, is minuscule enough to account for}, \addtxt{(9) availability of a large number of switchable loads within the distribution network connected at the transmission substation enables treating the sheddable loads as a continuous variable \cite{9019635}}, and \addtxt{(10) finite up- and down-time limits of the generators are ignored, especially when the event is in progress, and once disconnected, they will not be brought online until thorough risk assessment.} \sout{The solution, $V_{k}$ and the convergence status, $q_k$ of the optimization problem constitute the state of the power system, $s^{p}_{k}$ = \{$V_k \cup q_k$\}. However, its important to point out that the generator set points identified as a part of the solution of the optimization problem takes finite amount of time to manifest in the real world. Since the system model utilizes a discrete model of time with a relative large step size, we assume solution of the optimization problem as the part of power systems state at the current time step. (LAST ARGUMENT MIGHT NEED REVISION)}

\subsection{Modeling Wildfire Spread ($\mathcal{F}^{fire}$)}
\label{sec:wildfire}
\subsubsection{Wild-Fire Propagation in Topographical Space}
\input{fire_spread}

\subsubsection{Topography to Topology Mapping}
\label{sec:impact}
\Subir{This paragraph is moved to first paragraph of section 3}\change{An approaching wildfire can increase}{Increasing average ambient temperature} \change{of a cell that can cause internal faults in power system components}{due to approaching wildfire can result into sag, increasing the potential of faults for the power transmission lines. If a heavily loaded line is outaged, it is imminent that some of the lines can be overloaded, and subsequently cascaded outage may occur (as it was observed in 1977 New York black-out \cite{Time2015NewYork}). Therefore, it is critical from power system operational point of view not to remove any energized lines, especially when the power system operator is myopic and reactive, to avoid the possibility of cascading.} \sout{For instance, increase in temperature can melt the insulation causing two conductors coming in contact resulting in short circuit. Such faulty devices are isolated by the protection devices. This de-energizing effect is captured with the help of set of boolean variables.}

\addtxt{To realize the impact of propagating wildfire described in \ref{sec:wildfire}, the power system environment is geo-coded. Topologically,} \change{We view}{the} power system \addtxt{can be represented} as a collection of nodes, $N$, \addtxt{representing,} generation and transmission sub-stations, \sout{that are} connected through a set of transmission lines, $T$. For each node $n \in N$ and branch $t \in T$, we define corresponding boolean variables ($z_n^{f}, z_t^{f}$), to indicate their operational \change{state as a result of wildfire, i.e. True implies operational and False signifies non-operational}{status}. \addtxt{It is true that increasing temperature with approaching wildfire would result into derated operation of the transmission lines, as indicated in Section \ref{2.Assumptions}, we state inoperability of the transmission and generating assets when the wildfire is within certain proximity as identified by the variable $\mathcal{L}(s^x_k)$. Mathematically,} \sout{For each node and transmission line, the function, $\mathcal{F}^{map}$ returns True if all the cells, that the equipment spans over, are in \texttt{NOT\_IGNITED} state. It is formally defined as per Equation~\ref{eq:impact}}
\begin{equation}
        z_i^{f} = 
        \begin{cases}
        0 & \text{if} \quad  \exists x \in G_i \:\:\text{s.t.}\:\: \mathcal{L}(s^x_k) \ne \texttt{NOT\_IGNITED}  \\
        1 & \text{otherwise}
    \end{cases}
    \label{eq:impact}
\end{equation}
where the set $G_i$ \Subir{There is no discussion on how $G_i$ is calculated} contains the cells that the equipment, $i$ spans over. \change{The set cardinality, $\vert G_i \vert$ is greater than one for transmission lines whereas  $\vert G_i \vert$ equals to 1 for nodes. The set \{$z_n^f$  $\forall n \in N$ , $z_t^f$ $\forall t \in T$\} constitutes the internal control input, $u^{I}_k$ as}{As indicated in Figure~\ref{fig:blockdiagram}, $\lbrace z_n^f~\forall n \in N ,~z_t^f~\forall t \in T \rbrace$ constitutes the internal control input, $u^{I}_k$, representing the discussed emergency call or the overloading condition, received by the operator directly from the environment.}


\subsection{Simulated Power System Operation }
\label{sec:power}
In this section, \addtxt{in contrary with traditional power system operator conducting the multi-period optimization}, we \change{model the daily}{describe it as a reactive and myopic entity, actively seeking the recommendation of an external controller. The state of the power system at $k^{th}$ instant is already known to the operator. As discussed earlier, the operator receives the emergency responses, given by, $z_{n,k}^{f}$ and $z_{t,k}^{f}$, from various agencies (see, $\mathcal{F}^{map}$), and emergency substation and transmission line de-energization information from the external controller (given as, $z_{n,k}^{e}$ and $z_{t,k}^{e}$) at the $k^{th}$ instant and first deploys them judiciously. Consequently, the revised operational status of a substation or the line for the ${k+1}^{th}$ instant becomes $z^{o}_{i,k+1} = z_{i,k}^{e}z_{i,k}^{f}z^{o}_{i,k}$ and $z^{o}_{t,k+1} = z_{t,k}^{e}z_{t,k}^{f}z^{o}_{t,k}$ respectively.}\Subir{The way the variable $z$ has been used, it can be confusing to the reviewers. Add an identifier that separates generators, nodes, and lines.} 

\addtxt{The operator also utilizes the demand forecast along with rest of the information received from the external controller at the $k^{th}$ instant, and measured system state at the $k^{th}$ instant, to derive the complete list of set-points of the generators, and, load shedding schedule while aiming to minimize the value of lost load at the $k+1^{th}$ instant. Since this stage is done following topology update stage, we use derived system topology ($z^{o}_{i,k+1}, z^{o}_{t,k+1}$) in this regard. The consequent problem to be solved is given as:} \sout{ operations of the power system from the perspective of a system operator as mixed integer non-linear optimization problem, with an objective  to maximize the load delivery or minimize the load loss as described in Equation~\ref{eq:objective}}
\begin{equation*}
     \stkout{\min_{V_{k}} \sum_{i \in N} w^{c\_l}_i \Delta P^{c\_l}_{i,k} + w^{nc\_l}_i \Delta P^{nc\_l}_{i,k}  + w^{g} \big( P^{g}_{i,k} -  P^{g}_{i,k-1} \big)^2}
    % \label{eq:objective}
\end{equation*}

\begin{equation}
    \min_{V_{k+1}} \sum_{i \in N} w^{c\_l}_i \Delta P^{c\_l}_{i,k+1} + w^{nc\_l}_i \Delta P^{nc\_l}_{i,k+1}  + w^{g} \left( P^{g}_{i,k+1} -  P^{g}_{i,k} \right)^2
    \label{eq:objective}
\end{equation}

where \change{$V_k$}{$V_{k+1}$} \Subir{If not defined already, change $V_k$ to $\Phi_k$, and $w^{g}$ to $\epsilon$.} is the set of decision variables \addtxt{of the operator in the second stage,} that includes, power generation output\addtxt{s} \change{$P^{g}_{i,k}$}{$P^{g}_{i,k+1}$}, critical, non-critical load\addtxt{s} shedded \change{($\Delta P^{c\_l}_{i,k}$, $\Delta P^{nc\_l}_{i,k}$)}{($\Delta P^{c\_l}_{i,k+1}$, $\Delta P^{nc\_l}_{i,k+1}$)}, \change{voltage}{nodal} angle\addtxt{s} \change{$\theta_{i,k}$}{$\theta_{i,k+1}$}, operational state of \sout{the }generator\addtxt{s} \change{$z_i^o$}{group $z_{i,k+1}^g$} of node $i \in N$ \addtxt{(without any loss of generality, all the generators at a given bus are aggregated)} along with \sout{power}{line} flow\addtxt{s}, \change{$P^{flow}_{t,k}$}{$P^{flow}_{t,k+1}$}, through branch $t \in T$\sout{ as well as its operational status, $z^{o}_{t}$}. \change{Only specifying the load loss expression,}{Sole utilization of value of load loss expression as an objective,} \change{$\big( \Delta P^{c\_l}_{i,k} +  \Delta P^{nc\_l}_{i,k} \big)$}{$\sum_{i \in N} w^{c\_l}_i \Delta P^{c\_l}_{i,k+1} + w^{nc\_l}_i \Delta P^{nc\_l}_{i,k+1}$} \sout{in the objective function} \change{may lead to}{leads to the possibility of} multiple feasible solutions with undesirable \change{changes to power injections}{ramping of the generators (artifact of myopic nature of the operator)}. \change{However, the addition of the expression,}{Addition of an expression} \change{$\big( P^{g}_{i,k} -  P^{g}_{i,k-1} \big)^2$}{$\sum_{i \in N} \left( P^{g}_{i,k+1} -  P^{g}_{i,k} \right)^2$} \addtxt{with minuscule bias of $w^{g}$ prohibits such a condition, with little to no impact on the original objective function. The criticality of the loads (hospitals, fire stations, police stations, etc. are generally treated as critical loads) imposes the condition of $w^{c\_l}_i \geq w^{nc\_l}_i > 0$ ($\forall i \in N$). These values can be different for different nodes. Furthermore, $\min{w^{nc\_l}_i} \gg w^{g} > 0$. Determination of these weights are beyond the scope of this research, and is assumed to be known apriori.} \sout{encourages the solver to find a solution that avoid unnecessary ramping up or down of generators with little impact on the over-all load loss due to presence of the weights $w^{c\_l}_i $, $w^{nc\_l}_i$ and $w^{g}$ such that $w^{c\_l}_i > w^{nc\_l}_i > w^{g}$ $\forall i \in N$.}\addtxt{The nullity of the decision variable space $V_{k+1}$ indicates non-existance of the solution, indicating possible cascading, and is captured through variable $q_k$. The state of the power system is captured by $s^{p}_{k}$ = \{$V_k \cup q_k$\}. }

\change{The operator has to achieve the goal while adhering to safety constraints associated with different equipment even in the wake of changing operating conditions as a result of adverse weather effects such as wildfires etc. We classify these constraints into three categories as Generation, Load Demand and Load Flow constraints, defined as follows}{The discussed objective function must be subjected to the following power system operational and safety related constraints:}

\subsubsection{Generation Constraints}
\sout{These constraints are imposed due to} Finite generation capacity \addtxt{(given by, P$^{min}_i$, P$^{max}_i$)} and \sout{limited} ramping \sout{up or down }capabilities \addtxt{(given by, $\text{R}^{max}_{i}$) limit the operability} of the generators. \addtxt{These parameters are predefined positive real numbers. In this stage, the network topology has already been revised, and hence, we use $z^{o}_{i,k+1}$ to determine nodal availability. The external controller identifies the generator to be controlled, through $v^{e}_{i,k}$ ($\in u^{e}_{i,k}$), and also provides incremental set point adjustment, $\Delta P^{e}_{i,k}$. The operator, in return, checks the feasibility in terms of the upper limit of the received set-point (based on current operating state of the generators $z^{g}_{i,k}$) using \eqref{eq:in:su}, failing which the operator reports non-convergence through $q_{k+1}$. If the lower limit is violated through $z^{e}_{i,k}$ (see, \eqref{eq:in:su3}), the limits remain unchanged; otherwise, minimum and maximum operating limits of the generators ($\text{P}^{min,*}_i, \text{P}^{max,*}_i$) are updated using \eqref{eq:in:su1}-\eqref{eq:in:su2}.}

\begin{gather}
        0 \leq v^{e}_{i,k} \left( P^{g}_{i, k} + \Delta P^{e}_{i,k} \right) \leq v^{e}_{i,k} z^{o}_{i,k+1} z^{g}_{i,k} \text{P}^{max}_i \label{eq:in:su} \\
        z^{e}_{i,k} = \left\{\begin{matrix}
            0; ~~~\text{if}~~ v^{e}_{i,k} \left( P^{g}_{i, k} + \Delta P^{e}_{i,k} \right)  \leq v^{e}_{i,k} z^{o}_{i,k+1} z^{g}_{i,k} \text{P}^{min}_i \\ 
            1; ~~~~~~~~~~~~~~~~\text{otherwise}
                             \end{matrix}\right.   \label{eq:in:su3}\\
        \text{P}^{min,*}_i = z^{e}_{i,k} \left( P^{g}_{i, k} + \Delta P^{e}_{i,k} \right) +  (1 - z^{e}_{i,k}) \text{P}^{min}_i \label{eq:in:su1}\\
        \text{P}^{max,*}_i = z^{e}_{i,k} \left( P^{g}_{i, k} + \Delta P^{e}_{i,k} \right) +  (1 - z^{e}_{i,k}) \text{P}^{max}_i  \label{eq:in:su2}
\end{gather}

\addtxt{In a constantly changing environment, generators can suffer from forced outage (defined by, $z^{g}_{i,k+1}$), to avoid the system suffering from cascading failure, with the help of its load rejection capabilities \cite{4111968}. Therefore during this case, the generators ramping rate and operating limit can be allowed to breach (see, \eqref{eq:Gen_lim}), under the condition that once outaged they won't be brought online without through safety check. For the purpose of this paper, these generators will remain outaged indefinitely (see, \eqref{eq:zo}). We seek the help of a large positive real constant, $\Gamma^0$, in this regard. These conditions along with revised generating and ramping capability is given in the following equations. Here, $\Delta k$ represents the operating interval of the power system. }

\begin{gather}
        0 \leq z^{g}_{i,k+1} \leq z^{g}_{i,k} \label{eq:zo}\\
        z^{g}_{i,k+1} {\text{P}^{min,*}_{i}} \leq P^{g}_{i,k} \leq z^{g}_{i,k+1} {\text{P}^{max,*}_{i}} \label{eq:Gen_lim}\\
        -\Gamma^{0} \left(1-z^{g}_{i,k+1}\right) -\Delta k R^{max}_{i} \leq P^{g}_{i,k+1} - P^{g}_{i,k}~~~~~~~~~~~~~~~~~~~~~~~~~ \nonumber \\
        ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\leq \Delta k R^{max}_i + \Gamma^{0} \left(1-z^{g}_{i,k+1}\right) \label{eq:ramp_lim}
\end{gather}




\sout{Equation~\ref{eq:Gen_lim} forces the power generation, $P^{g}_{i,k}$ at node $i$ to be bounded by the lower and upper thresholds, (P$^{min}_i$, P$^{max}_i$), where $P^{g}_{i,k}$ is a real valued decision variable and (P$^{min}_i$, P$^{max}_i$) are constants. The boolean decision variable, $z^{o}_{i,k}$ captures the operational state of the node $i$ and guarantees $P^{g}_{i,k} = 0$ if the node is turned off. According to Equation~\ref{eq:zo}, $z^{o}_{i,k}$ depends upon the previous value, $z^{o}_{i, k-1}$, along with boolean variables, ($z^{f}_{i,k} \in u^{I}_{k}$, $z^{e}_{i,k} \in u^{E}_{k}$), where $u^{I}$ and $u^{E}$ represent the internal and external control input as shown in Figure~\ref{fig:blockdiagram}. Equation~\ref{eq:zo} implies that if a node, $i$ is deemed non-operational either due to wildfire ($z^{f}_{i,k}$), external stimuli ($z^{e}_{i,k}$) or operator action ($z^{o}_{i,k}$) at a time step $k$, then it remains non-operational for all future time steps i.e. $z^{o}_{i, k+1} = 0$. Equation~\ref{eq:ramp_lim} ensures the change in the power generation at node $i$ is bounded by a constant $\Delta k \text{R}^{max}_{i}$, where R$^{max}_i$ is the maximum ramp rate and $\Delta k$ is the step size. If the node is non-operational, then constraint in Equation~\ref{eq:ramp_lim} is relaxed by the addition of very large constant $\Gamma^0$, defined in Equation~\ref{eq:m}. The decision variable, $P^{g}_{i,k}$ is fixed to a value, $P^{g}_{i, k-1} + \Delta P^{e}_{i,k}$, provided by the external stimuli given the node is operational, $z^{o}_{i,k} = 1$ and the boolean variable, $v^{e}_{i,k} \in u^{e}_{i,k}$ is true, according to Equation~\ref{eq:in} where $v^{e}_{i,k}$ represents the exogenous variable for selecting a node to update the power generation by a fixed value. }
\begin{gather*}
   \stkout{     0 \leq z^{o}_{i,k} \leq z^{f}_{i,k} z^{e}_{i,k} z^{o}_{i,k-1}} \label{eq:zo:a}\\
   \stkout{     z^{o}_{i,k} {P^{min}_{i}} \leq P^{g}_{i,k} \leq z^{o}_{i,k} {P^{max}_{i}}} \label{eq:Gen_lim:a}\\
    \stkout{    -\Gamma_i -\Delta k R^{max}_{i} \leq P^{g}_{i,k} - P^{g}_{i,k-1} \leq \Delta k R^{max}_i + \Gamma_i} \label{eq:ramp_lim:a}\\
    \stkout{    \Gamma_i = \Gamma^{0} \big(1-z^{o}_{i,k}\big)}\label{eq:m:a}\\
    \stkout{    v^{e}_{i,k} P^{g}_{i,k} = v^{e}_{i,k} z^{o}_{i,k } \big( P^{g}_{i, k-1} + \Delta P^{e}_{i,k} \big)} \label{eq:in:a}
\end{gather*}

\subsubsection{Load Demand Constraints}
\addtxt{Restricted availability of local generation during contingencies necessitates curtailment of load demand.} \change{Due to removal of a node or a branch in the system, power flow has to be redistributed by changing the power injected at some of the nodes. If the load demand cannot be fulfilled by the generating stations, then part of the load has to be curtailed. We use a real valued variable,}{As defined in Section \ref{2.Assumptions}, suppose, P$^{l}_{i,k+1}$ is the operator predicted load demand, then, following removal of associated substation, updated load demand will be $z^{o}_{i,k+1}\text{P}^{l}_{i,k+1}$. Additionally, $\alpha_i$ is the critical load fraction (positive real number known apriori). Since the critical and non critical load fractions are treated as continuous variable, critical and non-critical sheddable loads ($\Delta P^{c\_l}_{i,k+1}, \Delta P^{nc\_l}_{i,k+1}$) is bounded as follows:} 

\begin{gather}
    0 \leq \Delta P^{c\_l}_{i,k+1} \leq \alpha_i z^{o}_{i,k+1} \text{P}^l_{i, k+1} \label{eq:Crit_lim:SM}\\
    0 \leq \Delta P^{nc\_l}_{i,k+1} \leq  (1 - \alpha_i) z^{o}_{i,k+1} \text{P}^l_{i,k+1} \label{eq:NCrit_lim:SM}
\end{gather}

\sout{$P^{l}_{i,k}$, to denote the available load at bus $i$ which is equal to its initial value, P$^{l}_{i,0}$ if the node $i$ is operational, otherwise 0 as per Equation~\ref{eq:availableload}. The load demand at every node can be classified into two broad groups, 1) Critical (hospitals, fire stations, police stations etc) and 2) Non-critical (residential). The load curtailment procedure should remove non-critical load followed by critical. We use two real valued decision variables, ($\Delta P^{c\_l}_{i,k}$, $\Delta P^{nc\_l}_{i,k}$) to denote amount of critical and non-critical load removed at node $i$. These variables are bounded by the available load as shown in Equations~\ref{eq:Crit_lim} and \ref{eq:NCrit_lim}, where $\alpha_i$ is the fraction of critical load present at node $i$.} 
\begin{gather*}
    \stkout{P^{l}_{i, k} = z^{o}_{i,k} \text{P}^l_{i, 0}} \label{eq:availableload}\\
    \stkout{0 \leq \Delta P^{c\_l}_{i,k} \leq \alpha_i P^l_{i, k}} \label{eq:Crit_lim}\\
    \stkout{0 \leq \Delta P^{nc\_l}_{i,k} \leq  (1 - \alpha_i) P^l_{i,k}} \label{eq:NCrit_lim}
\end{gather*}


\subsubsection{Load Flow Constraints}
\change{We utilize a DC load flow model~\cite{dcmodel} to represent power flow in the system extended with operational status of nodes and branches.}{Since the typical operating voltage within the power system remains close to 1.00 \textit{pu}, and the difference in the voltage angle of the adjacent buses are very small, we consider a DC power flow model \cite{stevenson1975element}; and the associated mathematical expression is given in \eqref{eq:Power_Flow_01:SM}. Here, B$_t$ is the element corresponding to the $t^{th}$ branch in the imaginary part of the nodal admittance matrix. Equation \eqref{eq:Node_Bal:SM} represents the nodal flow balance equation. Also, the set $T^{i} \subseteq T$ consists of all the branches that are connected to node $i$. Here, $\theta^{min}, \theta^{max}$ are nodal angle upper and lower bound. The power flow constraint is described in \eqref{eq:line_therm:SM}.} 

\begin{gather}
    P^{g}_{i,k+1}  - P^l_{i,k+1}z^{o}_{i,k+1} + \Delta P^{c\_l}_{i,k+1} + \Delta P^{nc\_l}_{i,k+1} \nonumber \\ 
    ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~- \sum_{t \in T^i} P^{flow}_{t,k+1} = 0 \label{eq:Node_Bal:SM} \\
    P^{flow}_{t,k+1} -  z^{o}_{t,k+1} \text{B}_{t} \left( \theta_{i,k+1} - \theta_{j,k+1} \right)  = 0 \label{eq:Power_Flow_01:SM} \\
    \theta^{min} \leq \theta_{i,k+1} \leq \theta^{max} \label{eq:angle_lim:SM} \\
    - z^{o}_{t,k+1} \text{P}^{maxflow}_{t}  \leq P^{flow}_{t,k+1} \leq z^{o}_{t,k+1} {\text{P}^{maxflow}_{t}} \label{eq:line_therm:SM}
\end{gather}

\sout{Equation~\ref{eq:Node_Bal} captures the nodal power balance at $i$, where the real valued decision variable, $P^{flow}_{t,k}$ denotes the power flowing through the branch $t$ connected to node $i$. The set $T^{i} \subseteq T$ consists of all the branches that are connected to node $i$. Equation~\ref{eq:Power_Flow_01} determines the power flow in the line $t \in T^{i}$ between nodes $i, j \in N$, where B$_t$ is the susceptance of the line and $\theta_i$ is the voltage angle at node $i$. The power flowing through a line is constrained by the thermal power rating as described in Equation~\ref{eq:line_therm}, where P$^{maxflow}_t$ denotes the maximum power that can flow through a line and $z^{o}_{t,k}$ denotes the operational state of the line. If the line is removed as a result of wildfire or external input, then $z^{o}_{t,k} = 0$ as per Equation~\ref{eq:beta} and forces the power flowing through line, $P^{flow}_{t,k} = 0$ in both Equations~\ref{eq:Power_Flow_01}  and~\ref{eq:line_therm}. } \Subir{It will be wrong to call B-matrix as the susceptance matrix.}




\begin{gather*}
    \stkout{z^{o}_{t,k} =  z^{f}_{t,k} z^{e}_{t,k} z^{o}_{t, k-1}}\label{eq:beta}\\
    \stkout{P^{g}_{i,k}  - P^l_{i,k} + \Delta P^{c\_l}_{i,k} + \Delta P^{nc\_l}_{i,k} - \sum_{t \in T^i} P^{flow}_{t,k} = 0} \label{eq:Node_Bal} \\
    \stkout{P^{flow}_{t,k} -  z^{o}_{t,k} \text{B}_{t} \big( \theta_{i,k} - \theta_{j,k} \big)  = 0} \label{eq:Power_Flow_01} \\
    \stkout{\theta^{min} \leq \theta_{i,k} \leq \theta^{max}} \label{eq:angle_lim} \\
    \stkout{- z^{o}_{t,k} \text{P}^{maxflow}_{t}  \leq P^{flow}_{t,k} \leq z^{o}_{t,k} {\text{P}^{maxflow}_{t}}} \label{eq:line_therm}
\end{gather*}


% \subsection{Assumptions}
% System model depends upon the following assumptions, 1) Wildfire propagation model assumes the effect of geographical factors such as terrain slope and type along with environmental factors such as wind velocity and humidity etc are implicitly captured by P$^{x}_{y,k}$ and is known before hand. 2) The power system operations model assumes the load demand at every node remains constant. 3) The solution, $V_{k}$ and the convergence status, $q_k$ of the optimization problem constitute the state of the power system, $s^{p}_{k}$ = \{$V_k \cup q_k$\}. However, its important to point out that the generator set points identified as a part of the solution of the optimization problem takes finite amount of time to manifest in the real world. Since the system model utilizes a discrete model of time with a relative large step size, we assume solution of the optimization problem as the part of power systems state at the current time step. (LAST ARGUMENT MIGHT NEED REVISION)

 
% \subsection*{}
% As shown in Figure~\ref{fig:blockdiagram}, the output, $s^{p}_k$ of the function, $f^{power}$ depends upon output of the previous step, $s^{p}_{k-1}$ and control inputs, $u^{I}_k$, $u^{E}_k$ The state of the power system, $s^{p}_k$ at time step $k$ is a tuple, \{$q_k$, $P^{g}_{i,k}$, $\Delta P^{c\_l}_{i,k}$, $\Delta P^{nc\_l}_{i,k}$, $\theta_i$, $z_{i,k}^o$, $P^{flow}_{j,k}$ \} $\forall i \in N$, $\forall j \in T$, where $P^{g}_i$ represents power generated at node $i$, ($P^{c\_l}_i$, $P^{nc\_l}_i$) captures the critical and non-critical load curtailed at node $i$, ($\theta^i$, $z_i^o$) signify the voltage angle and operational status of node $i$, $P^{flow}_k$ denote the power flowing through branch $j$ and $q$ represents the convergence status. The external control input, $u^{E}_k$, includes set of boolean variables, \{ $z_{n,k}^{e}$, $z_{t,k}^{e}$, $v_{n,k}^{e}$ \} for each node, $n \in N$ and branch $t \in T$ in power system along with set of real variables, $\Delta P^{e}_{n,k}\:\: \forall n \in N$. The boolean variables, ($z_{n,k}^{e}$, $z_{t,k}^{e}$) represent the operational state of the node and branches as instructed by external stimulus. True value of the boolean variable, $v_{n,k}^{e}$ denotes generation at the  node $n$ to be updated by a real variable, $\Delta P^{e}_{n,k}$.
% The function, $f^{power}$ is modeled as a mixed integer non-linear program with the objective to minimize the load loss as defined in Equation~\ref{eq:objective}




==> 3_problem_formulation.tex <==
\section{Problem Formulation}\label{SecFormulation}

{\color{red}Define optimal control policy formally (this is what RL will try to approximate).}

\Subir{Seek the help of one of the earlier draft to complete.}

The RL agent, based on the observation from the fire propagation model and power system operational state $s_{t}$, determine actions to be taken in terms of removal of lines, $\Delta E_{t}$, and providing set points to some of the generators. Nullity of $\Phi_{t+1}$ is driven by set-points provided to some of the generators, and operation of transmission lines, during previous time intervals. Furthermore, if the agent provides an infeasible set of operating points to the power system operator, then also, $\Phi_{t+1} = \varnothing$.

The topological condition of the system will be a function of both action of the protection devices induced by the fire event and line removal command provided by the agent, which can be given by the following set of equations: 

\begin{gather}
    E_{t+1} = E_{t}\setminus \left( \Delta E_{t} \cup \Delta' E_{t}\right ) \\
\delta_{i,j,t+1} = \left\{\begin{matrix}
1, & (i,j) \in E_{t}\setminus \left( \Delta E_{t} \cup \Delta' E_{t}\right ) \\ 
0, & \text{otherwise}
\end{matrix}\right. \\
V_{t+1} = V_{t}\setminus \left( \Delta V_{t} \cup \Delta' V_{t}\right ) \\
\psi_{i,t+1} = \left\{\begin{matrix}
1, & i \in V_{t+1} \\ 
0, & \text{otherwise}
\end{matrix}\right.
\end{gather}

Here, $\Delta E_{t}$ and $\Delta V_{t}$ are line and substation removal command, respectively, provided by the agent, and $\Delta' E_{t}$, and $\Delta' V_{t}$ are the set of lines and substations that are isolated due to fire. Additionally, operating on energized nodes or lines can be perilous. Therefore, such an operation will be heavily penalized. These conditions are obtained through the variable $\mathcal{L}^{H,NF,O}_{t+1}$. The penalty will be even larger, if either of $\Delta E_{t} \cup \Delta' E_{t}$ and $\Delta V_{t} \cup \Delta' V_{t}$ are non-null, i.e., operational devices are struck by fire, independent of their energization status. If such a condition appears, those devices will be immediately opened through the operation of the protection devices. This condition is represented using $\mathcal{L}^{H,F,O}_{t+1}$. The energization status of the substations can be calculated by the absolute sum of the power flow, and associated conditions are given by $\mathcal{N}^{H,NF,O}_{t+1}$ and $\mathcal{N}^{H,F,O}_{t+1}$ respectively. Please note that the operational status of generators gets directly accounted for in this process.


\begin{gather}
\mathcal{L}^{H,F,O}_{t+1} = \left\lbrace 1, \exists (i,j) \in \Delta' E_{t} \cap E_{t} \left| \left|P^{Line}_{i,j,t}\right| > 0    \right.  \right\rbrace  \\
\mathcal{L}^{H,NF,O}_{t+1} = \begin{Bmatrix}
1,  \exists (i,j) \in \Delta E_{t} \cap E_{t} \left|    \left|P^{Line}_{i,j,t}\right| > 0 \right. \\ 
~~ ~ \land ~\Delta' E_{t} \cap E_{t} = \varnothing    
\end{Bmatrix} \\
\mathcal{N}^{H,F,O}_{t+1} = \begin{Bmatrix}
1, \exists i \in \Delta' V_{t} \cap V_{t}\\ 
~~\left|  \sum_{\forall j \in V_{t}} \left|P^{Line}_{i,j,t}\right| > 0    \right.
\end{Bmatrix} \\
\mathcal{N}^{H,NF,O}_{t+1} = \begin{Bmatrix}
1,  \exists i \in \Delta E_{t} \cap E_{t} \left|    \sum_{\forall j \in V_{t}} \left|P^{Line}_{i,j,t}\right| > 0 \right.\\ 
~~ ~ \land ~\Delta' E_{t} \cap E_{t} = \varnothing    
\end{Bmatrix}
\end{gather}

We calculate the reward function for the current set of actions provided by the agent as follows:

\begin{equation}
r(t+1) = \left\{\begin{matrix}
\mathcal{P}'', ~\text{if}~~\Phi_{t+1} = \varnothing \\
\mathcal{P}' -  \left(\rho^C \bm{\Delta P^{C,L}_{t+1}} + \rho^{NC} \bm{\Delta P^{NC,L}_{t+1}}\right), \\ 
\text{if}~\left( \mathcal{L}^{H,F,O}_{t+1} = 1 \lor \mathcal{N}^{H,F,O}_{t+1} = 1 \right) \land \Phi_{t+1} \neq \varnothing\\ \mathcal{P} -  \left(\rho^C \bm{\Delta P^{C,L}_{t+1}} + \rho^{NC} \bm{\Delta P^{NC,L}_{t+1}}\right), \\ 
\text{if}~\left( \mathcal{L}^{H,NF,O}_{t+1} = 1 \lor \mathcal{N}^{H,NF,O}_{t+1} = 1\right)  \land \Phi_{t+1} \neq \varnothing \\
-   \left(\rho^C \bm{\Delta P^{C,L}_{t+1}} + \rho^{NC} \bm{\Delta P^{NC,L}_{t+1}} \right), ~\text{otherwise}
\end{matrix}\right.
\end{equation}

As discussed, it is imperative that $\mathcal{P}'' \ll \mathcal{P}' \ll \mathcal{P} \ll 0$.


\Aron{express objective as optimizing rewards over future timesteps with temporal discounting}

==> 4_drl.tex <==
\section{Deep Reinforcement Learning (DRL) Based Proactive Control}
    \input{rl_procedure/0_overview}
    % \input{rl_procedure/1_types_of_agents}
    \input{rl_procedure/2_rl_agent}
    % \input{rl_procedure/3_training}


==> problem_formulation_aj.tex <==
\section{Problem Formulation}
\label{sec:Formulation}

\change{An approaching wildfire can increase}{Increasing average ambient temperature} \change{of a cell that can cause internal faults in power system components}{due to approaching wildfire can result into sag, increasing the potential of faults for the power transmission lines. If a heavily loaded line is outaged, it is imminent that some of the other energized lines can be overloaded, and subsequently cascaded outage may occur (as it was observed in 1977 New York black-out \cite{Time2015NewYork}). Therefore, it is critical from power system operational point of view to avoid removal of any energized line/ substation, especially when the power system operator is myopic and reactive, to avoid the possibility of cascading.} \sout{For instance, increase in temperature can melt the insulation causing two conductors coming in contact resulting in short circuit. Such faulty devices are isolated by the protection devices. This de-energizing effect is captured with the help of set of boolean variables.}


\change{The behavior of the power system operator described in previous section is myopic in nature i.e. it tries to redistribute the flow of power in the system to achieve maximum load delivery for the next time step. This short sighted horizon may lead to series of control actions that are}{Sole utilization of the reactive, and consequent myopic, system operator may lead to multi-period} sub-optimal \change{for the system's future}{operation} \change{trajectory}{of the system}. \change{Moreover, the response of the operator to the effects of wildfire is reactive as it tries to redistribute the power after node or a branch has been deemed non-operational by the wildfire. Lastly, removal of number of energized power system equipment due to action of either protection devices or operator can shift the system towards instability resulting in cascading outages.}{Therefore, the external controller bears an enormous amount of responsibility, to predict future trajectory of the system, and provide appropriate control signal, vis-\'a-vis, prevent the system from running into possible cascading.} \sout{There is a need of a supplementary controller that can suggest proactive actions to the operator and aid in making better decisions to manage the effects of wildfire by taking into account the prospective trajectories of the wildfire propagation and its effect on the power system equipment. (THIS MIGHT NEED REVISION: SHORTENING)} \addtxt{Here, w}e formulate the control problem as a Markov Decision Problem (MDP) and refer to as $\mathcal{D}$. A MDP is a tuple, \{$S$, $A$, $\mathcal{P}_a(s,s')$, $\mathcal{R}_a$\}, where $S$ is a finite state space, $A$ is a finite action space, $\mathcal{P}_a(s,s')$ is the probability that action $a \in A$ in state $s \in S$ will lead to state $s' \in S$ and $\mathcal{R}_a(s,s')$ is the reward received when action $a \in A$ is taken in state $s \in S$ to reach $s' \in S$. For $\mathcal{D}$, these elements are defined as follows\addtxt{:}

\textbf{States:} At any time step $k$, the state of $\mathcal{D}$ is defined by a tuple, \{$s^{f}_k$, $s^{p}_k$\} where $s^{f}_k$ is the state of wildfire in the grid and $s^{p}_k$ is the state of power system described in previous section. The complete state space, $S$ is defined as $S \subseteq \{0,1\}^{M + \vert T \vert + \vert N \vert +1 } \times \mathbb{R}^{M + \vert T \vert + 3\vert N \vert}$, where $M$ \Subir{Note that, $\mathrm{M}$ and $M$ are different symbols. Please be consistent.} is the number of cells in the grid and ($\vert N \vert$, $\vert T \vert$) are the numbers of nodes and branches in the system. 


\textbf{Actions:} The decision problem can control operational state of nodes and branches, $z^{e}_{i}, z^{e}_{i} \in u^{E}$ and change power injections at nodes using $v^{e}_i$, $\Delta P^{e}_{i}\in u^{E}$. The action space, $A$ is defined as $A \subseteq \{0,1\}^{2\vert N \vert + \vert T \vert} \times \mathbb{R}^{\vert N \vert}$

\textbf{Transitions:} A MDP evolves as a result of actions taken and new states reached. For $\mathcal{D}$, representing the transition probability explicitly is difficult. We utilize the episodic simulation of the system model, described in Figure~\ref{fig:blockdiagram} as an implicit model of $\mathcal{D}$. An episodic simulator can be started from an initial state and yields a subsequent state every time it receives an action input. The sequence of states, action inputs constitutes an episode.

\textbf{Reward Function:} 
Since the objective of $\mathcal{D}$ is \sout{to maximize the load delivery} \Subir{please do not introduce new terms, which may lead to errors.} while minimizing the impact of wildfire on power system operations and maintaining all constraints \Subir{since, MDP itself is solving another optimization problem, the use of the word constraints can be confusing}, we define a reward function \Subir{Please use the revised text to rewrite the reward function in a concise fashion}, $\mathcal{R}_a(s_{k-1},s_{k})$ that imposes penalties if the new state, $s'$, incurs a load loss, ($r_1$), contains removal of energized equipment as a result of action $a$, ($r_2$)  or wildfire, ($r_3$)  and is undefined due to non-convergence i.e. unable to satisfy at least one of the constraints, ($r_4$)  as described in Equation~\ref{eq:total}.

\begin{gather}
        \mathcal{R}_a(s_{k-1}, s_k) \:=\:  r_1 + r_2 +  r_3 + r_4\label{eq:total}\\
        r_1 = -q_k \sum_{i \in N} P^{l}_{i,0} - P^{l}_{i,k} + \Delta P^{c\_l}_{i,k} + \Delta P^{nc\_l}_{i,k}\label{eq:loadloss}\\
        r_2 = -q_k \bigg( \sum_{i \in N} \psi^{e}_{i,k} \vert P^{g}_{i,k-1} \vert + \sum_{t \in T}  \psi^{e}_{t,k} \vert P^{flow}_{t,k-1} \vert \bigg) \label{eq:active}\\
      r_3 = -q_k \bigg( \sum_{i \in N}  \psi^{f}_{i,k} P^{l}_{0} +  \sum_{t \in T}  \psi^{f}_{t,k}P^{l}_{0} \bigg) \label{eq:wildfire}\\ 
      r_4 = (\vert N \cup T \vert) (q_k - 1)P^{l}_{0} \label{eq:constraints}
\end{gather}

Equation~\ref{eq:loadloss} defines the load loss penalty, $r_1$, where the expression $P^{l}_{i,0} - P^{l}_{i,k}$ \Subir{Use brackets judiciously} signifies the load loss due to removal of node and $\Delta P^{c\_l}_{i,k} + \Delta P^{nc\_l}_{i,k}$ denotes the load curtailed by the optimization problem. The active equipment removal penalty is equal to the power flowing through the branch or power injected at the node as defined in Equation~\ref{eq:active}, where $\psi^{e}_{j,k} = (z^{o}_{j, k-1} \oplus z^{e}_{j,k})$ denotes the change in the operational status of the equipment, $j \in \{N \cup T\}$ as a result of action input. $\psi^{e}_{j,k}$ evaluates to True if equipment $j$ was operational in $k-1^{th}$ time step but non-operational in the current time step, $k$.\footnote{The expression, $(z^{o}_{j, k-1} \oplus z^{e}_{j,k})$ can evaluate to True if the equipment was non-operational in the previous time-step but operational now. However, this is not possible due to constraints defined in Equations~\ref{eq:zo} and~\ref{eq:beta}.} The wildfire penalty, $r_3$ is equal to the total initial load, P$^l_0$ in the system as defined in Equation~\ref{eq:wildfire}, where $\psi^{f}_{j,k} = (z^{o}_{j, k-1} \oplus z^{f}_{j,k})$ denotes the change in the operational status of the equipment, $j \in \{N \cup T\}$ as a result of wildfire. The non-convergence penalty, defined in Equation~\ref{eq:constraints} equals to initial load value times the number of equipment in the system. The non-convergence penalty, $\vert r_4 \vert$ is the highest followed by the wildfire penalty, $\vert r_3 \vert$ as the decision process must learn to satisfy all system safety constraints and the high value of wildfire penalty ensures that the decision process provides pro-active measures and should not allow wild-fire to come in contact with an energized equipment.



\textbf{Policy:} A policy, $\pi(s)$ is a function that specifies the action to be taken in the state $s \in S$. The goal of solving a MDP is to find a policy that maximises the cumulative sum of expected rewards that the decision problem generates as a result of following the said policy, defined in Equation~\ref{eq:policy}, where $\gamma \in [0,1]$ is the discount factor.

\begin{equation}
    \pi_a = \max\: \mathbb{E}[ \sum_{k=0}^{\infty} \gamma^k \mathcal{R}_a(s_k, s_{k+1})] \label{eq:policy}
\end{equation}
(ARON/ ABHISHEK/ SALAH : NEED HELP WITH THIS EQUATION)

% \begin{equation}
%     \begin{aligned}
%         \mathcal{R}_a(s_k, s_{k+1}) =&  w_1 r_1 + w_2 r_2 +  w_3 r_3 + w_4 r_4\\
%         r_1 =& -q_k \sum_{i \in N} P^{l}_{i,0} - P^{l}_{i,k} + \Delta P^{c\_l}_{i,k} + \Delta P^{nc\_l}_{i,k}\\
%         r_2 =& -q_k \sum_{i \in N} (z^{o}_{i, k-1} \oplus z^{f}_{i,k}) \vert P^{g}_{i,k-1} \vert \\&+  \sum_{t \in T} (z^{o}_{t, k-1} \oplus z^{f}_{t,k}) \vert P^{flow}_{t,k-1} \vert\\
%       r_3 =& -q_k \sum_{i \in N} (z^{o}_{i, k-1} \oplus z^{e}_{i,k}) \vert P^{g}_{i,k-1} \vert \\&+  \sum_{t \in T} (z^{o}_{t, k-1} \oplus z^{e}_{t,k})\vert P^{flow}_{t,k-1} \vert\\ 
%       r_4 =& (\vert N \vert + \vert T \vert) \sum_{i \in N}  (q_k - 1)P^{l}_{i, 0}
%     \end{aligned}
% \end{equation}


% \begin{equation}
%     \begin{gathered}
%         \mathcal{R}_a(s_k, s_{k+1}) \:=\:  r_1 + r_2 +  r_3 + r_4\\
%         r_1 = -q_k \sum_{i \in N} P^{l}_{i,0} - P^{l}_{i,k} + \Delta P^{c\_l}_{i,k} + \Delta P^{nc\_l}_{i,k}\\
%         r_2 = -q_k \bigg( \sum_{i \in N} (z^{o}_{i, k-1} \oplus z^{e}_{i,k}) \vert P^{g}_{i,k-1} \vert + \sum_{t \in T} (z^{o}_{t, k-1} \oplus z^{e}_{t,k}) \vert P^{flow}_{t,k-1} \vert \bigg) \\
%       r_3 = -q_k \bigg( \sum_{i \in N} (z^{o}_{i, k-1} \oplus z^{f}_{i,k}) P^{l}_{i,0} +  \sum_{t \in T} (z^{o}_{t, k-1} \oplus z^{f}_{t,k})P^{l}_{i,0} \bigg) \\ 
%       r_4 = (\vert N \cup T \vert) \sum_{i \in N}  (q_k - 1)P^{l}_{i, 0}
%     \end{gathered}
% \end{equation}


% \begin{align}
%     &\mathcal{R}_a(s_k, s_{k+1}) =  r_1 + r_2 +  r_3 + r_4 \label{eq:total}\\
%     &r_1 = -q_k \sum_{i \in N} P^{l}_{i,0} - P^{l}_{i,k} + \Delta P^{c\_l}_{i,k} + \Delta P^{nc\_l}_{i,k}\label{eq:loadloss}\\
%     &r_2 = -q_k \bigg( \sum_{i \in N} (z^{o}_{i, k-1} \oplus z^{e}_{i,k}) \vert P^{g}_{i,k-1} \vert \quad+\nonumber\\&\qquad\qquad\qquad \sum_{t \in T} (z^{o}_{t, k-1} \oplus z^{e}_{t,k}) \vert P^{flow}_{t,k-1} \vert \bigg) \label{eq:active}\\
%     &r_3 = -q_k \bigg( \sum_{i \in N} (z^{o}_{i, k-1} \oplus z^{f}_{i,k}) P^{l}_{i,0} \quad+ \nonumber\\ &\qquad\qquad\qquad  \sum_{t \in T} (z^{o}_{t, k-1} \oplus z^{f}_{t,k})P^{l}_{i,0} \bigg) \label{eq:wildfire}\\ 
%     &r_4 = (\vert N \cup T \vert) \sum_{i \in N}  (q_k - 1)P^{l}_{i, 0} \label{eq:constraints}
% \end{align}

==> test_results/2_rl_agent.tex <==

\subsection{Implementation Procedure of the Proactive/RL Agent}
We want an agent that can take the right actions proactively. For that agent, we first need to choose the right algorithm.

% \Aron{motivate why we use RL instead of some online approach, such as MCTS}
% \Salah{This section is for the implementation procedure. I think the section name was misleading, so I've change it. Please, let me know if we still want to add motivation here or somewhere else. }


% \Aron{also, mention in the results section that the execution (one step) of the trained policy takes only a fraction of a second}

\subsubsection{Choosing an algorithm}
The agent uses the observation as input and generates action as output. In this experiment, the action space and the observation space are pretty large, and several fields contain continuous values as well. The decision mainly depends on the fire distance from the equipment (power system's nodes, transmission lines, and generators) and the current status of that equipment regardless of time or place. So, we can consider an off-policy algorithm for the agent that also supports continuous action space. Explicitly, we consider the Deep Deterministic Policy Gradient (DDPG)~\cite{lillicrap2015continuous} algorithm for the agent.
% \Aron{motivate choice of DDPG}
The algorithm is a model-free, off-policy actor-critic algorithm using deep function approximators that can learn policies in high-dimensional, continuous action spaces.

The DDPG algorithm combines the idea of the Deterministic Policy Gradient (DPG) algorithm with the Deep Q Network (DQN). In general, the algorithm uses the actor-network to generate action and the critic-network for the value or reward function. The agent applies the action to the environment that returns a negative reward (penalty) for improper action. The agent updates its network based on the critic generated penalty and the penalty from the environment. The algorithm also uses a target actor and critic network to provide consistency in the network. It uses a replay buffer to store the records, a record is a tuple of state, action, reward and next state, and trains the network by sampling a random fixed-size mini-batch from the buffer. 


\subsubsection{Agent implementation}
The agent needs to shut off buses and branches if there is a fire and set the ramp values of the generators accordingly. Shutting off buses or branches depends upon external weather impacts. So, we do not allow switching on once a bus or branch is shut off. But, it restricts the exploration area of the RL agents. Moreover, shutting off buses or branches is not a continuous action where the ramp values are continuous actions. The DDPG algorithm is ideal for continuous action spaces. 

On the other side, it is possible to make decisions to shut off buses and branches based on fire distance. The agent can simply switch off the bus or branch when the fire is at a minimum safe distance. The agent does not need a neural network to make the decision. 

Setting a ramp value is not as easy as shutting off buses or branches. We cannot use a heuristic rule to set the ramp values. It depends on many factors of the power system and which is complex. After considering all things, we decide to use the heuristic rule to switch off buses and branches and a neural network to set the ramp values.



\subsubsection{Complexity analysis of the neural network}
The agent needs to make decisions for the ramp values. Ideally, the agent could select several generators and set the ramp values to that generator when it is necessary. But, selecting generators and setting the ramp values is a two-layer problem. Even before learning the original problem (setting the ramp values), the agent needs to learn the relation between these two-layer. So, if there is n number of generators, and the agent needs to select k number of generators, then the agent actually needs to select a possible way out of $\Mycomb[n+k-1]{k}$ different ways. Here, the neural network may select the same generator multiple times during selecting k generators as we cannot restrict the output. As an example, if we have 10 generators, and the agent needs to select 5 generators to set the ramp values, then the agent needs to select a possible way out of 2,002 different ways. So, if we simply use a neural network for selecting generators and their corresponding ramp values, then it would be very tough for the neural network to learn all the possible ways, and their ramp values and finding the best one.

To solve the issue, we follow two different ways. The agent selects all the generators and sets the ramp up, down, or zero values in every time step. In this case, the agent controls all the generators and the total power generation. Here, the number of possible ways of selecting generators is 1. At this time, the agent needs to work only on setting the ramp values. It does not need to learn the relation between selecting generators with the ramp values. The downside is that the power system operator cannot help to optimize the power generation. We call this approach a \textit{full-control agent}.

On the other hand, we can create several mini-groups and assign a small number of generators to each group. The agent will select a generator from each group, and set the ramp values. The remaining generators will be controlled by the power system operator. So, if there are m groups and every group is consists of k generators, where k is a small number, then the agent needs to select a possible way out of $k^m$. Now, let's return back to the previous example and create 5 groups and assign 2 generators in each group. Based on the neural network output, the agent selects a generator from each group. The agent sets ramp up, down, or zero values for 5 generators and the other 5 generators are free for the power system operator. Here, the agent needs to learn a possible way out of 32. In this case, the agent partially controls the power generation. We call this approach a \textit{partial-control agent}.  

Note here, we use GAMS as the power system operator. The operator changes the ramp values to reduce the load losses. However, if the agent sets the ramp value for a generator, then the system operator does not change the value for that generator by itself. So, we expand our experiments by training the agent for both ways. 


\subsubsection{Set generators initial output as maximum output}
The agent needs to generate a valid action that converges in the environment. An action converges if it satisfies all the constraints, otherwise the agent will get a violation penalty with a termination for that episode. In the beginning, it is obvious to have a lot of violation penalty for its large action space where the decided action is random. We set initial power generation as maximum power generation to reduce the number of violations at the beginning. We assume the power system is settled and the power demand cannot be increased. Although, a power generator may need to increase the power generation if there is a fire in another generator. However, for the sake of reducing the number of violations and speeding up the training, we set the initial power generation as the maximum power generation. 


\subsubsection{Mapping to original power generation output}
We notice that it works better if the neural network produces the power generation output instead of producing directly the ramp values. We can easily calculate the ramp values from the neural network generated output and the generator's original output. It seems that this way works better because the input values (observation) are more related to the power generation output than the ramp values. 


 






==> test_results/base_case/base_case.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            xmax=100,
            xlabel = Episode,
            ylabel = Penalty
            ]
            \addplot table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/base_case/base_case.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Base case episode vs penalty}
    \label{fig:base_case}
\end{figure}




total penalty,-> individual component penalty





==> test_results/base_case/base_case_hist.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=20pt,
            % xmax=100,
            xlabel={Penalty},
            ylabel={Percentage},
            % ytick=\empty,
            % nodes near coords*={\pgfmathprintnumber\pgfplotspointmeta\%}
            ]
            \addplot +[
            hist={
                bins=100,
            }   
        ] table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/base_case/base_case.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Base case episode vs penalty}
    \label{fig:my_label}
\end{figure}

==> test_results/base_case/heuristic_fire_distance_with_base_case.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            xmax=100,
            xlabel = Episode,
            ylabel = Penalty
            ]
            \addplot table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/base_case/heuristic_fire_distance_with_base_case.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties after applying actions based on fire distance}
    \label{fig:heuristic_fire_distance_with_base_case}
\end{figure}

==> test_results/base_case/heuristic_fire_distance_with_base_case_hist.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=20pt,
            % xmax=100,
            xlabel={Penalty},
            ylabel={Percentage},
            % ytick=\empty,
            % nodes near coords*={\pgfmathprintnumber\pgfplotspointmeta\%}
            ]
            \addplot +[
            hist={
                bins=100,
            }   
        ] table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/base_case/heuristic_fire_distance_with_base_case.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties after applying actions based on fire distance}
    \label{fig:my_label}
\end{figure}

==> test_results/episodic_analysis/general_case/active_line_removal.tex <==

\begin{figure}
\centering

\begin{tikzpicture}
  \def\basis{1}
  \pgfplotsset
    {
    y coord trafo/.code={\pgfmathparse{symlog(#1,\basis)}\pgfmathresult},
    y coord inv trafo/.code={\pgfmathparse{symexp(#1,\basis)}\pgfmathresult},
    yticklabel style={/pgf/number format/.cd, int detect, precision=0},
    }
    
    \begin{axis}[
        xlabel={Step},
        ylabel={Cumulative active line removal penalty},
        line width=0.05cm,
        legend style={at={(.66,.1)},anchor=west}
    ]
    
    \addlegendentry{proactive}
    \addplot [sharp plot, red] table[x=step, y=active_line_removal, col sep=comma]
    {test_results/episodic_analysis/general_case/proactive_cumulative.csv};
    
    \addlegendentry{reactive}
    \addplot [sharp plot, blue] table[x=step, y=active_line_removal, col sep=comma] {test_results/episodic_analysis/general_case/reactive_cumulative.csv};
    
    \end{axis}
\end{tikzpicture}
\caption{Episodic active line removal penalty over every step}
\label{fig:general_case_episodic}
\end{figure}



==> test_results/episodic_analysis/general_case/load_loss.tex <==

\begin{figure}
\centering

\begin{tikzpicture}
  \def\basis{1}
  \pgfplotsset
    {
    y coord trafo/.code={\pgfmathparse{symlog(#1,\basis)}\pgfmathresult},
    y coord inv trafo/.code={\pgfmathparse{symexp(#1,\basis)}\pgfmathresult},
    yticklabel style={/pgf/number format/.cd, int detect, precision=0},
    }
    
    \begin{axis}[
        xlabel={Step},
        ylabel={Cumulative load loss penalty},
        line width=0.05cm,
        legend style={at={(.66,.1)},anchor=west}
    ]
    
    \addlegendentry{proactive}
    \addplot [sharp plot, red] table[x=step, y=load_loss, col sep=comma]
    {test_results/episodic_analysis/general_case/proactive_cumulative.csv};
    
    \addlegendentry{reactive}
    \addplot [sharp plot, blue] table[x=step, y=load_loss, col sep=comma] {test_results/episodic_analysis/general_case/reactive_cumulative.csv};
    
    \end{axis}
\end{tikzpicture}
\caption{Episodic load loss over every step}
\label{fig:general_case_episodic}
\end{figure}



==> test_results/episodic_analysis/general_case/total_penalty.tex <==

\begin{figure}
\centering

\begin{tikzpicture}
%   \def\basis{1}
%   \pgfplotsset
%     {
%     y coord trafo/.code={\pgfmathparse{symlog(#1,\basis)}\pgfmathresult},
%     y coord inv trafo/.code={\pgfmathparse{symexp(#1,\basis)}\pgfmathresult},
%     yticklabel style={/pgf/number format/.cd, int detect, precision=0},
%     }
    
    \begin{axis}[
        xlabel={Step},
        ylabel={Total penalty},
        % line width=0.01cm,
        legend style={at={(.33,.91)},anchor=east}
    ]
    
    \addlegendentry{proactive}
    \addplot [sharp plot, red] table[x=step, y=total_penalty, col sep=comma]
    {test_results/episodic_analysis/general_case/proactive_cumulative.csv};
    
    \addlegendentry{reactive}
    \addplot [sharp plot, blue] table[x=step, y=total_penalty, col sep=comma] {test_results/episodic_analysis/general_case/reactive_cumulative.csv};
    
    \end{axis}
\end{tikzpicture}
\caption{Total penalty over every step in an example episode.}
\label{fig:general_case_episodic}
\end{figure}



==> test_results/episodic_analysis/general_case/wildfire.tex <==

\begin{figure}
\centering

\begin{tikzpicture}
  \def\basis{1}
  \pgfplotsset
    {
    y coord trafo/.code={\pgfmathparse{symlog(#1,\basis)}\pgfmathresult},
    y coord inv trafo/.code={\pgfmathparse{symexp(#1,\basis)}\pgfmathresult},
    yticklabel style={/pgf/number format/.cd, int detect, precision=0},
    }
    
    \begin{axis}[
        xlabel={Step},
        ylabel={Cumulative wildfire penalty},
        line width=0.05cm,
        legend style={at={(.66,.1)},anchor=west}
    ]
    
    \addlegendentry{proactive}
    \addplot [sharp plot, red] table[x=step, y=wildfire, col sep=comma]
    {test_results/episodic_analysis/general_case/proactive_cumulative.csv};
    
    \addlegendentry{reactive}
    \addplot [sharp plot, blue] table[x=step, y=wildfire, col sep=comma] {test_results/episodic_analysis/general_case/reactive_cumulative.csv};
    
    \end{axis}
\end{tikzpicture}
\caption{Episodic wildfire penalty over every step}
\label{fig:general_case_episodic}
\end{figure}



==> test_results/episodic_analysis/non_convergence.tex <==

\begin{figure}
\centering

\begin{tikzpicture}
%   \def\basis{1}
%   \pgfplotsset
%     {
%     y coord trafo/.code={\pgfmathparse{symlog(#1,\basis)}\pgfmathresult},
%     y coord inv trafo/.code={\pgfmathparse{symexp(#1,\basis)}\pgfmathresult},
%     yticklabel style={/pgf/number format/.cd, int detect, precision=0},
%     }
    
    \begin{axis}[
        xlabel={Step},
        ylabel={Cumulative penalty},
        % line width=0.05cm,
        mark repeat=25,
        legend style={at={(1.0,1.25)},anchor=east}
    ]
    
    % \addlegendentry{load loss (reactive)}
    \addplot [sharp plot, blue] table[x=step, y=load_loss, col sep=comma] {test_results/episodic_analysis/non_convergence/reactive_cumulative.csv};

    % \addlegendentry{load loss (proactive)}
    \addplot [sharp plot, red] table[x=step, y=load_loss, col sep=comma]
    {test_results/episodic_analysis/non_convergence/proactive_cumulative.csv};
    
    % \addlegendentry{wildfire (reactive)}
    \addplot [sharp plot, blue, dashed] table[x=step, y=wildfire, col sep=comma] {test_results/episodic_analysis/non_convergence/reactive_cumulative.csv};

    % \addlegendentry{wildfire (proactive)}
    \addplot [sharp plot, red, dashed] table[x=step, y=wildfire, col sep=comma]
    {test_results/episodic_analysis/non_convergence/proactive_cumulative.csv};
    
    % \addlegendentry{active line removal (reactive)}
    \addplot [sharp plot, blue, dotted, thick] table[x=step, y=active_line_removal, col sep=comma] {test_results/episodic_analysis/non_convergence/reactive_cumulative.csv};

    % \addlegendentry{active line removal (proactive)}
    \addplot [sharp plot, red, dotted, thick] table[x=step, y=active_line_removal, col sep=comma]
    {test_results/episodic_analysis/non_convergence/proactive_cumulative.csv};
    
    \end{axis}
\end{tikzpicture}
\caption{Different types of penalty components over every step in an example episode (ending in non-convergence for reactive).}
\label{fig:penalty_component_nc_example}
\end{figure}



==> test_results/episodic_analysis/non_convergence/load_loss.tex <==
\begin{figure}
\centering


\begin{tikzpicture}
\def\basis{1}
\pgfplotsset
{
y coord trafo/.code={\pgfmathparse{symlog(#1,\basis)}\pgfmathresult},
y coord inv trafo/.code={\pgfmathparse{symexp(#1,\basis)}\pgfmathresult},
yticklabel style={/pgf/number format/.cd,int detect,precision=0},
}
\begin{axis}[
        xlabel={Step},
        ylabel={Cumulative load loss penalty},
        % ymode=log,
        % ymin=0,
        % xmin=0,
        line width=0.05cm,
        legend style={at={(.66,.1)},anchor=west}
    ]
    
    \addlegendentry{proactive}
    \addplot[sharp plot, red] table[x=step, y=load_loss, col sep=comma] {test_results/episodic_analysis/non_convergence/proactive_cumulative.csv};

    \addlegendentry{reactive}
    \addplot[sharp plot, blue] table[x=step, y=load_loss, col sep=comma]
    {test_results/episodic_analysis/non_convergence/reactive_cumulative.csv};
\end{axis}
\end{tikzpicture}
\caption{Episodic load loss penalty over every step (non-convergence)}
\label{fig:general_case_episodic}
\end{figure}

==> test_results/episodic_analysis/non_convergence/total_penalty.tex <==
\begin{figure}
\centering


\begin{tikzpicture}
\def\basis{1}
\pgfplotsset
{
y coord trafo/.code={\pgfmathparse{symlog(#1,\basis)}\pgfmathresult},
y coord inv trafo/.code={\pgfmathparse{symexp(#1,\basis)}\pgfmathresult},
yticklabel style={/pgf/number format/.cd,int detect,precision=0},
}
\begin{axis}[
        xlabel={Step},
        ylabel={Cumulative total penalty},
        % ymode=log,
        % ymin=0,
        % xmin=0,
        line width=0.01cm,
        legend style={at={(.66,.1)},anchor=west},
        % restrict y to domain=0:1000
        width=\columnwidth
    ]
    
    \addlegendentry{proactive}
    \addplot[sharp plot, red] table[x=step, y=total_penalty, col sep=comma] {test_results/episodic_analysis/non_convergence/proactive_cumulative.csv};

    \addlegendentry{reactive}
    \addplot[sharp plot, blue] table[x=step, y=total_penalty, col sep=comma]
    {test_results/episodic_analysis/non_convergence/reactive_cumulative.csv};
\end{axis}
\end{tikzpicture}
\caption{Total penalty over every step in an example episode (ending in non-convergence for reactive).}
\label{fig:general_case_episodic}
\end{figure}

==> test_results/full_control_over_power_generation/fixed_fire_source.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            xmax=100,
            xlabel = Episode,
            ylabel = Penalty
            ]
            \addplot table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/full_control_over_power_generation/fixed_fire_source.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties for fixed fire source (controlling full power generation)}
    \label{fig:fixed_fire_full_control}
\end{figure}

==> test_results/full_control_over_power_generation/fixed_fire_source_hist.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=20pt,
            xmax=-60000,
            xmin=-220000,
            % xmax=100,
            xlabel={Penalty},
            ylabel={Percentage},
            % ytick=\empty,
            % nodes near coords*={\pgfmathprintnumber\pgfplotspointmeta\%}
            ]
            \addplot +[
            hist={
                bins=100,
            }   
        ] table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/full_control_over_power_generation/fixed_fire_source.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties for fixed fire source (controlling full power generation)}
    \label{fig:my_label}
\end{figure}

==> test_results/full_control_over_power_generation/random_fire_source.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            xmax=100,
            xlabel = Episode,
            ylabel = Penalty
            ]
            \addplot table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/full_control_over_power_generation/random_fire_source.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties for random fire source (controlling full power generation)}
    \label{fig:random_fire_full_control}
\end{figure}

==> test_results/full_control_over_power_generation/random_fire_source_hist.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=20pt,
            xmax=-60000,
            xmin=-220000,
            xlabel={Penalty},
            ylabel={Percentage},
            % ytick=\empty,
            % nodes near coords*={\pgfmathprintnumber\pgfplotspointmeta\%}
            ]
            \addplot +[
            hist={
                bins=100,
            }   
        ] table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/full_control_over_power_generation/random_fire_source.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties for random fire source (controlling full power generation)}
    \label{fig:my_label}
\end{figure}

==> test_results/partial_control_over_power_generation/fixed_fire_source.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            xmax=100,
            xlabel = Episode,
            ylabel = Penalty
            ]
            \addplot table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/partial_control_over_power_generation/fixed_fire_source.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties for fixed fire source (controlling partial power generation)}
    \label{fig:fixed_fire_partial_control}
\end{figure}

==> test_results/partial_control_over_power_generation/fixed_fire_source_hist.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=20pt,
            xmax=-60000,
            xmin=-220000,
            xlabel={Penalty},
            ylabel={Percentage},
            % ytick=\empty,
            % nodes near coords*={\pgfmathprintnumber\pgfplotspointmeta\%}
            ]
            \addplot +[
            hist={
                bins=100,
            }   
        ] table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/partial_control_over_power_generation/fixed_fire_source.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties for fixed fire source (controlling partial power generation)}
    \label{fig:my_label}
\end{figure}

==> test_results/partial_control_over_power_generation/fixed_fire_source_load_loss.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=20pt,
            xmax=-60000,
            xmin=-220000,
            xlabel={Penalty},
            ylabel={Percentage},
            % ytick=\empty,
            % nodes near coords*={\pgfmathprintnumber\pgfplotspointmeta\%}
            ]
            \addplot +[
            hist={
                bins=100,
            }   
        ] table [x=episode_number, y=load_loss, col sep=comma]     {test_results/partial_control_over_power_generation/fixed_fire_source.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties for fixed fire source (controlling partial power generation)}
    \label{fig:my_label}
\end{figure}

==> test_results/partial_control_over_power_generation/random_fire_source_hist.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=20pt,
            % xmax=-60000,
            % xmin=-220000,
            xlabel={Penalty},
            ylabel={Percentage},
            % ytick=\empty,
            % nodes near coords*={\pgfmathprintnumber\pgfplotspointmeta\%}
            ]
            \addplot +[
            hist={
                bins=100,
            }   
        ] table [x=episode_number, y=total_penalty, col sep=comma]     {test_results/partial_control_over_power_generation/random_fire_source.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties for random fire source (controlling partial power generation)}
    \label{fig:my_label}
\end{figure}

==> test_results/partial_control_over_power_generation/random_fire_source_load_loss.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=20pt,
            % xmax=-60000,
            % xmin=-220000,
            xlabel={Penalty},
            ylabel={Percentage},
            % ytick=\empty,
            % nodes near coords*={\pgfmathprintnumber\pgfplotspointmeta\%}
            ]
            \addplot +[
            hist={
                bins=100,
            }   
        ] table [x=episode_number, y=load_loss, col sep=comma]     {test_results/partial_control_over_power_generation/random_fire_source.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Penalties for random fire source (controlling partial power generation)}
    \label{fig:my_label}
\end{figure}

==> test_results/spaces_and_penalties.tex <==
% \subsection{Spaces and penalties}
% The agent needs to ramps up or down the power generation of generators based on different situations. The agent also needs to shut off buses or branches if there is a fire. The agent acts in every time step based on current observation and receives reward accordingly.


% \subsubsection{Action spaces}
% There are four fields in the action space. In our test environment, we have 24 nodes (buses), 34 transmission lines (branches), and 11 power generators. To minimize the impact of the external weather event, we want to shut off the nodes or the transmission lines before the event hits them. In the action space, we use binary arrays to set the status of nodes and transmission lines whether we want to keep them alive or shutdown. We need to de-energize the nodes and the transmission lines before changing their status from living to shut off. So, we need to reduce the power supply from the generators. In the action space, we have defined an integer array to select the power generators and another floating-point array to set the ramping up or down power for the corresponding generators.


% \subsubsection{Observation space}
% To make the decision in each action, the environment simulator provides the current status (observation) to the agent. We define six fields in the observation space. Nodes and the transmission line's status are binary arrays, like the action space, that describes the current state of each component. We define a floating-point array with the size of the number of nodes and the transmission lines to get the information (distance) of fire from each component. The agent also gets information about the amount of power that flows through the transmission lines. For generators, we use an integer array to select the generators and floating-point arrays to get the current output of corresponding generators and theta values. 


% \subsubsection{Penalties}
% In every time step, the agent acts and receives penalties accordingly. We define four types of penalties and the agent receives a summation of all the penalties if it is not a violation penalty. 

% A violation happens when the taken action cannot be converged in the simulator or the GAMS during solving the optimization problem. We don't want to get this penalty at any cost. So, we define a very high penalty for this type of action. We calculate the violation penalty in the following way. 

% $violation\_penalty = -10*number\_of\_components*total\_power\_demand$

% There are in total of 58 components (24 buses, 34 branches), and the total initial power demand is 2850 MW. So, for a non-convergence action, the agent receives a constant value of -1,653,000 unit penalty. 

% We define a no action is taken or a protection penalty if there is a fire in a component of the power system, but the agent does not take any action. 

% $protection\_penalty = -2 * total\_power\_demand$

% So, this is a constant value which incurs in a total of -5700 unit of penalty.

% The third type of penalty that we define is the active line removal penalty. If the agent removes an active line from the power system, then the agent receives a penalty of equivalent to the amount of power was flowing through that line. 

% The last type of penalty that we define is the load loss penalty. If there is a demand of power is x MW, but the power system generates a power of y MW which is smaller than x, then the agent will receive a penalty of $-1*(x-y)*system\_base\_MVA$ unit penalties. The system base MVA is a constant value of 100. 

% In every time step, the agent receives a penalty based on its action. If there is no violation in the action, then the agent receives a penalty of summation of all other penalties. 

% \begin{algorithmic}
% \IF {$action\_converge$} 
%         \STATE $return (protection\_penalty * number\_of\_occurrence + 
%         active\_line\_removal\_penalty * number\_of\_occurrence + 
%         load\_loss\_penalty)$
% \ELSE
%         \STATE $return\ non\_convergence\_penalty$
% \ENDIF 
% \end{algorithmic}

